Adversarial Machine Learning Threat Analysis and Remediation in Open Radio Access Network (O-RAN)

O-RAN is a new, open, adaptive, and intelligent RAN architecture. Motivated by the success of artificial intelligence in other domains, O-RAN strives to leverage machine learning (ML) to automatically and efficiently manage network resources in diverse use cases such as traffic steering, quality of experience prediction, and anomaly detection. Unfortunately, it has been shown that ML-based systems are vulnerable to an attack technique referred to as adversarial machine learning (AML). This special kind of attack has already been demonstrated in recent studies and in multiple domains. In this paper, we present a systematic AML threat analysis for O-RAN. We start by reviewing relevant ML use cases and analyzing the different ML workflow deployment scenarios in O-RAN. Then, we define the threat model, identifying potential adversaries, enumerating their adversarial capabilities, and analyzing their main goals. Next, we explore the various AML threats associated with O-RAN and review a large number of attacks that can be performed to realize these threats and demonstrate an AML attack on a traffic steering model. In addition, we analyze and propose various AML countermeasures for mitigating the identified threats. Finally, based on the identified AML threats and countermeasures, we present a methodology and a tool for performing risk assessment for AML attacks for a specific ML use case in O-RAN.

==> prolog-language.tex <==

\makeatletter

% initialisation of user macros
\newcommand\PrologPredicateStyle{}
\newcommand\PrologVarStyle{}
\newcommand\PrologAnonymVarStyle{}
\newcommand\PrologAtomStyle{}
\newcommand\PrologOtherStyle{}
\newcommand\PrologCommentStyle{}

% useful switches (to keep track of context)
\newif\ifpredicate@prolog@
\newif\ifwithinparens@prolog@

% save definition of underscore for test
\lst@SaveOutputDef{`_}\underscore@prolog

% local variables
\newcount\currentchar@prolog

\newcommand\@testChar@prolog%
{%
  % if we're in processing mode...
  \ifnum\lst@mode=\lst@Pmode%
    \detectTypeAndHighlight@prolog%
  \else
    % ... or within parentheses
    \ifwithinparens@prolog@%
      \detectTypeAndHighlight@prolog%
    \fi
  \fi
  % Some housekeeping...
  \global\predicate@prolog@false%
}

% helper macros
\newcommand\detectTypeAndHighlight@prolog
{%
  % First, assume that we have an atom.
  \def\lst@thestyle{\PrologAtomStyle}%
  % Test whether we have a predicate and modify the style accordingly.
  \ifpredicate@prolog@%
    \def\lst@thestyle{\PrologPredicateStyle}%
  \else
    % Test whether we have a predicate and modify the style accordingly.
    \expandafter\splitfirstchar@prolog\expandafter{\the\lst@token}%
    % Check whether the identifier starts by an underscore.
    \expandafter\ifx\@testChar@prolog\underscore@prolog%
      % Check whether the identifier is '_' (anonymous variable)
      \ifnum\lst@length=1%
        \let\lst@thestyle\PrologAnonymVarStyle%
      \else
        \let\lst@thestyle\PrologVarStyle%
      \fi
    \else
      % Check whether the identifier starts by a capital letter.
      \currentchar@prolog=65
      \loop
        \expandafter\ifnum\expandafter`\@testChar@prolog=\currentchar@prolog%
          \let\lst@thestyle\PrologVarStyle%
          \let\iterate\relax
        \fi
        \advance \currentchar@prolog by 1
        \unless\ifnum\currentchar@prolog>90
      \repeat
    \fi
  \fi
}
\newcommand\splitfirstchar@prolog{}
\def\splitfirstchar@prolog#1{\@splitfirstchar@prolog#1\relax}
\newcommand\@splitfirstchar@prolog{}
\def\@splitfirstchar@prolog#1#2\relax{\def\@testChar@prolog{#1}}

% helper macro for () delimiters
\def\beginlstdelim#1#2%
{%
  \def\endlstdelim{\PrologOtherStyle #2\egroup}%
  {\PrologOtherStyle #1}%
  \global\predicate@prolog@false%
  \withinparens@prolog@true%
  %\bgroup\aftergroup\endlstdelim%  % commented to remove additional brackets at the end of the listing when using the breakline option
}

% language name
\newcommand\lang@prolog{Prolog-pretty}
% ``normalised'' language name
\expandafter\lst@NormedDef\expandafter\normlang@prolog%
  \expandafter{\lang@prolog}

% language definition
\expandafter\expandafter\expandafter\lstdefinelanguage\expandafter%
{\lang@prolog}
{
  language            = Prolog,
  keywords            = {},      % reset all preset keywords
  showstringspaces    = false,
  alsoletter          = (,
  alsoother           = @$,
  moredelim           = **[is][\beginlstdelim{(}{)}]{(}{)},
  MoreSelectCharTable =
    \lst@DefSaveDef{`(}\opparen@prolog{\global\predicate@prolog@true\opparen@prolog},
}

% Hooking into listings to test each ``identifier''
\newcommand\@ddedToOutput@prolog\relax
\lst@AddToHook{Output}{\@ddedToOutput@prolog}

\lst@AddToHook{PreInit}
{%
  \ifx\lst@language\normlang@prolog%
    \let\@ddedToOutput@prolog\@testChar@prolog%
  \fi
}

\lst@AddToHook{DeInit}{\renewcommand\@ddedToOutput@prolog{}}

\makeatother
%
% --- end of ugly internals ---


% --- definition of a custom style similar to that of Pygments ---
% custom colors
\definecolor{PrologPredicate}{RGB}{000,031,255}
\definecolor{PrologVar}      {RGB}{024,021,125}
\definecolor{PrologAnonymVar}{RGB}{000,127,000}
\definecolor{PrologAtom}     {RGB}{186,032,032}
\definecolor{PrologComment}  {RGB}{063,128,127}
\definecolor{PrologOther}    {RGB}{000,000,000}

% redefinition of user macros for Prolog style
\renewcommand\PrologPredicateStyle{\color{PrologPredicate}}
\renewcommand\PrologVarStyle{\color{PrologVar}}
\renewcommand\PrologAnonymVarStyle{\color{PrologAnonymVar}}
\renewcommand\PrologAtomStyle{\color{PrologAtom}}
\renewcommand\PrologCommentStyle{\itshape\color{PrologComment}}
\renewcommand\PrologOtherStyle{\color{PrologOther}}

% custom style definition 
\lstdefinestyle{Prolog-pygsty}
{
  language     = Prolog-pretty,
  upquote      = true,
  stringstyle  = \PrologAtomStyle,
  commentstyle = \PrologCommentStyle,
  literate     =
    {:-}{{\PrologOtherStyle :-}}2
    {,}{{\PrologOtherStyle ,}}1
    {.}{{\PrologOtherStyle .}}1
}

% global settings
\lstset
{
  numbers=left,
  breaklines=true,
  captionpos = below,
  columns    = fullflexible,
  basicstyle = \scriptsize\ttfamily,
  frame      = lines,
  xleftmargin= 17pt,
  aboveskip=-2pt,
  belowskip=-15pt
}

==> sections/D_sections/4_E_General_Attacks.tex <==
\subsection{Attack Techniques \label{subsec:attack_tech}}
In this section, we review various attack techniques against ML systems.
A table summarizing the reviewed attacks is presented in Appendix~\ref{tab:attack_techniques}.\\

\begin{figure}[t]
            \centering
            \includegraphics[width=0.5\textwidth]{sections/figures/attack_tech.pdf}
             \caption{General attack techniques}
            \label{fig:aml_at}
\end{figure}

\noindent\textbf{Evasion attacks \label{subsubsec:evasion_attacks}} 
In evasion attacks the adversary exploits the ML model \textit{[F9]} by generating a crafted input sample (an adversarial example) which is very similar to some other correctly classified input but is incorrectly classified by the ML model.
The adversary's main objective is to compromise the integrity \textit{[AG1]} of the ML model \textit{[F9]} by causing the ML system to provide incorrect outputs for a specific input \textit{[T1]}. 
Evasion attacks can be broadly classified based on the following criteria: attack technique, which characterizes the technique used by the attacker to craft the adversarial example (e.g., gradient-based, boundary-based, and transferability-based); the threat model, which characterizes the attacker’s access capabilities and attacker's knowledge of the ML-based system  (e.g., white-box, black-box); and the attack's specificity, which characterizes the goal of the attacker (e.g., targeted vs untargeted).


\noindent\textbf{Poisoning attacks \label{subsubsec:poisoning_attacks}} 
In poisoning attacks, the adversary exploits the ML training procedure \textit{[F8]}, by injecting crafted data samples into the dataset used for training the learning algorithm \textit{[AG2]}.
The adversary main objective is either compromising the availability \textit{[AG2]} of the ML model \textit{[A9]} by causing the ML system to deploy a corrupted model \textit{[T2]}; or compromising the integrity \textit{[AG1]} of the ML model \textit{[F9]}, by causing the ML system to deploy a model, which provides wrong outputs on a specific input \textit{[T1]}.
Poisoning attacks can be generally classified based on the following criteria: attack technique, which characterizes the technique used by the attacker to craft the malicious input samples (i.e., gradient-based, if the attack is based on a gradient optimization method; and transferability-based, if the attack utilizes the transferability property of ML models); threat model, which characterizes the attacker’s access capabilities and the attacker's knowledge regarding the system (e.g., white-box and black-box), attack's specificity, which characterizes the goal of the attacker (i.e., targeted, if the attack aims to cause misclassification of a specific set of samples; or indiscriminate, if the attack aims to cause misclassification of any sample), and error specificity, which characterizes the type of error in multiclass problems (i.e., error-specific, if the attacker aims to have a sample misclassified as a specific class; or error-generic, if the attacker aims to have a sample misclassified as any of the classes other than the true class).


\noindent\textbf{Inference attacks \label{subsubsec:inference_attacks}}
In inference attacks (such as membership inference \textit{[T3]}, data property inference \textit{[T4]}, data reconstruction \textit{[T5]}, and model reconstruction \textit{[T6]}), the adversary exploits the ML model \textit{[F9]} to expose private information and thereby compromise the privacy \textit{[AG3]} of the ML model \textit{[F9]} or the data used to train it \textit{[F1],[F5]}.




==> sections/D_sections/4_F_Attack_Implementations.tex <==
\subsection{Attack Techniques and Implementations in \oran \label{subsec:attack_impl}}

\noindent \textbf{[AT1] Gradient-based white-box evasion attacks (targeted and untargeted).} An adversary with perfect knowledge about the model \textit{[AKM1]} deployed within the RIC (\nrt~or \nonrt) who has a UE \textit{[ACD4]} such as third-party infrastructure software provider or an \oran's software developer, can manipulate an input sample for the deployed model and craft it in such way that the classification loss is maximized. The manipulation is determined by the calculations of the classification loss's gradients with respect to the input sample~\cite{goodfellow2014explaining,kurakin2016adversarial,carlini2017adversarial}. For example, in the FGSM attack~\cite{goodfellow2014explaining}, the adversarial example is calculated by adding noise to the input sample, in the direction of the gradient of the classification loss with respect to the input sample.

\noindent \textbf{[AT2]} An adversary with knowledge about the task of the model deployed within the RIC (\nrt~or \nonrt), has access to the model's probabilities vector and has a UE such as an adversary that posses a UE and performs a malicious activity, can craft an adversarial sample for the deployed model, using model's gradients estimations, and cause the \mlaa~ to select a wrong E2 action.

\noindent \textbf{[AT3]} An adversary with knowledge about the task of the model deployed within the RIC (\nrt~or \nonrt), has access to model's decision and has a UE such as an adversary that posses a UE and performs a malicious activity, can craft an adversarial sample for the deployed model, using model's gradients estimation (using Monte Carlo methods), and cause the \mlaa~to select a wrong E2 action.

\noindent \textbf{[AT4]} An adversary with knowledge about the training dataset's property distribution and the task of the model deployed within the RIC (\nrt~or \nonrt), has access to model's decision and has a UE such as an adversary that posses a UE and performs a malicious activity, can craft an adversarial sample for the deployed model, using gradients calculations on a surrogate model trained on a surrogate data, and cause the \mlaa~to select a wrong E2 action.

\noindent \textbf{[AT5]} An adversary with knowledge about the training data the task of the model deployed within the RIC (\nrt~or \nonrt), has access to model's decision and has a UE such as an adversary that posses a UE and performs a malicious activity, can craft an adversarial sample for the deployed model, using gradients calculations on a surrogate model trained on the same data used to train the model, and cause the \mlaa~to select a wrong E2 action.

\noindent \textbf{[AT6]} An adversary with perfect knowledge about the model deployed within the RIC(\nrt~or \nonrt), who has access to write into the training data and has a UE such as third-party infrastructure software provider or an \oran's software developer, can inject crafted data samples into the training data and cause a miss-classification of some required data (error-specific) or corrupt the model classification performances in general (error-generic), therefore cause the \mlaa~to select a wrong E2 actions for future inputs.

\noindent \textbf{[AT7]} An adversary with knowledge about the training dataset's property distribution and the task of the model deployed within the RIC (\nrt~or \nonrt), has access to write into the training data and has a UE such as a third-party infrastructure software provider or an \oran's software developer, can inject crafted data samples into the training data and cause a miss-classification of some required data (error-specific) or corrupt the model classification performances in general (error-generic), therefore cause the \mlaa~to select a wrong E2 actions for future inputs.

\noindent \textbf{[AT10]} An adversary with perfect knowledge about the model deployed within the RIC (\nrt~or \nonrt), has access to write into the training data, and has a UE such as third-party infrastructure software provider or an \oran's software developer, can inject crafted data samples into the training data and cause a miss-classification of some required data (error-specific) or corrupt the model classification performances in general (error-generic), therefore cause the \mlaa~to select a wrong E2 action for future inputs.

\noindent \textbf{[AT11]} An adversary with knowledge about the training dataset's property distribution and the task of the model deployed within the RIC (\nrt~or \nonrt), has access to write into the training data and has a UE such as a third-party infrastructure software provider or an \oran's software developer, can inject crafted data samples into the training data and cause a miss-classification of some required data (error-specific) or corrupt the model classification performances in general (error-generic), therefore cause the \mlaa~to select a wrong E2 action for future inputs.

\noindent \textbf{[AT16]} An adversary with partial knowledge about the training data and the task of the model deployed within the RIC (\nrt~or \nonrt), has access to the model's probabilities vector and partial access to the model such as third-party infrastructure software provider or an \oran's software developer, can train a meta-classifier that can infer whether a model's training-set preserves a certain property and use it to learn information about the training dataset's property distribution.

\noindent \textbf{[AT17]} An adversary with partial knowledge about the training data and the task of the model deployed within the RIC (\nrt~or \nonrt), has access to the model's probabilities vector and partial access to the training data such as third-party infrastructure software provider or an \oran's software developer, can use Maximum a Posterior (MAP) estimation for the data and cause a leakage of samples from the training data and lead to data reconstruction and privacy violation.

\noindent \textbf{[AT18]} An adversary with perfect knowledge about the model deployed within the RIC (\nrt~or \nonrt) and the training data, has access to the model's probabilities vector and the training data such as third-party infrastructure software provider or an \oran's software developer, can use gradients calculations to recover samples from the training data and lead to data reconstruction and privacy violation.

\noindent \textbf{[AT19]} An adversary with limited knowledge about the task of the model deployed within the RIC (\nrt~or \nonrt), has access to the model's probabilities vector such as third-party infrastructure software provider, \oran's software developer or even an adversary that posses a UE and performs a malicious activity, can use an autoencoder settings where the decoder is trained on the deployed model's probabilities vector and reconstruct the training data and cause a privacy violation.

\noindent \textbf{[AT20]} An adversary with partial knowledge about the training data, the task and the algorithm of the model deployed within the RIC (\nrt~or \nonrt), has access to the model's probabilities vector such as third-party infrastructure software provider, \oran's software developer or even an adversary that posses a UE and performs a malicious activity, can create a substitute model that behaves very similar to the deployed model and cause a privacy issue and model extraction.

==> sections/D_sections/9_secassessexample.tex <==
\section{\label{sec:secexample} 
Example of Threat Assessment}

In this section we present a threat assessment of a specific machine learning-based application in O-RAN -- \emph{traffic steering}.
Based on the threat mapping of a general ML usecase in \oran, presented in Sections~\ref{sec:ontology} - \ref{sec:attack_tech}, we define a procedure and a tool that can be utilized for conducting the risk assessment of a specific usecase.

The risk assessment is conducted according to the following procedure:
\begin{enumerate}
\item \textbf{Provide title and description --} Provide the title and short description of the usecase (see Figure~\ref{fig:tsriskassessment}).

\item \textbf{Select threat actor --} Select the deployment scenario (out of the five possible deployment scenarios presented in Section~\ref{sec:ml_dep_oran}) as well as the threat actor (out of the six threat actors defined in Section~\ref{subsec:threatactor}), for which the risk assessment is conducted.
For example, in Figure~\ref{fig:tsriskassessment}, we can see that for the traffic steering use case, the selected deployment scenario is $DS2$, and the risk assessment is conducted for the malicious UE(s) threat actor ($[A5]$).

\item \textbf{Rank impact --} Rank the impact of each of the seven threat categories (defined in Section~\ref{sec:threat_category}) for the selected use case -- in our case, the traffic steering.
As can be seen in Figure~\ref{fig:tsriskassessment}, the selected impact for $[T1]$, which refers to the an attack that causes the model to provide incorrect output/s for a \emph{specific} input/s selected by the attacker, is `Medium' since it will result in specific, targeted users that will receive higher/lower quality of service when they should receive lower/higher quality of service (i.e., the impact on the provider is limited).

\item \textbf{Map capabilities and constraints to the analyzed use case --} In this step, we map the threat actor capabilities (access and knowledge) and additional constraints for the specific use case (i.e., traffic steering). 
This is done by grading several questions (presented in Figure~\ref{fig:tsriskassessment}), where each question is mapped to a specific capability. 
For example, $Q1$ in Figure~\ref{fig:tsriskassessment} refers to the capability of an attacker to manipulate the sensor/raw data of the ML use case. 
In the traffic steering use case, it is `Easy' for a malicious UE threat actor to manipulate the sensor/raw data since the sensors and raw data include signal information from the UEs and cells. 
Since the UEs are not trusted, an attacker can use malicious UEs and manipulate the signals. 
Each grade is mapped to a numeric score (according to a predefined scale).

\item \textbf{Map required capabilities and impacts to attack technique --} For each attack technique presented in Section~\ref{sec:attack_tech}, we map the capabilities that are required by the attacker.
This mapping is presented in Table~\ref{tab:attack_techniques_with_actors}.
For example, as can be seen in Table~\ref{tab:attack_techniques_with_actors}, the first attack technique, Gradient-based, white box evasion attack (such as C\&W, FGSM, PGD) requires full knowledge about the training data as well as the attacked model.
It also requires sensor data access in order to manipulate the adversarial samples. 
The possible impact of the attack in `Tempering', \i.e., causing the model to provide incorrect output/s for a specific input/s.
In addition, we assign for each attack technique a score that reflect the effectiveness of the performance of the adversarial attack technique.
This score ranking is derived based on the performance of the attack technique as reported in previous research.
This ranking is shown in Figure~\ref{fig:attackmapping}.
Note, that this mapping in performed once and it is use case-agnostic.

\item \textbf{Compute risk --} Based on information provided in steps (1)-(5), we can derive the risk for each attack technique within the specific use case (i.e., traffic steering). 
An example of the resulted risk for partial list of attack techniques is presented in Figure~\ref{fig:tsriskassessmenttechnique}.
The risk is the multiplication of the ranked impact (step (3)) and the likelihood of the attack and the effectiveness of the attack.
The likelihood of the attack is computed as the average of numeric scores of the attacker capabilities that are required by the attack technique (according to the mapping in step (5)).

\item \textbf{Prioritize threats --} Finally, based on the derived risk in step (6), we prioritize the threats for the selected use case (i.e., traffic steering).
The prioritized list is presented in Figure~\ref{fig:attackprioritization}.
As can be seen, the threat with the highest risk score is a malicious UE threat actor executing attack technique $AT4.1$ -- Gradient-based, white box poisoning attacks.
This is with high risk score (7.90) since the threat actor has access to the model as well as the ability to poison the model.
In addition, the impact of this attack (model corruption) is high and results in wrong prediction for any input.

\item \textbf{Select countermeasures --} In this last step, in order to mitigate the high risk threats, we can utilize the countermeasure ontology that is presented in Section~\ref{sec:countermeasures} for selecting the proper countermeasures.
The best countermeasure(s) can be selected first by their ability to mitigate the threat, and then by considering the use case requirements (e.g., impact on model performance, run time overhead), and the ability to apply the countermeasures in the specific use case.
For example, for mitigating the threat with the highest risk, possible countermeasures are data sensitization, data denoising, or using auxiliary models such as an AML detector in order to detect the poisoned samples.

\end{enumerate}



\begin{figure*}[h!]
    \centering
    \includegraphics[trim={1.5cm 1.5cm 2.5cm 0},clip, width=0.99\textwidth]{sections/figures/riskanalysis.pdf}
    \caption{Presenting the form that is used by the security domain expert for defining the threat actor capabilities and contraints for the selected usecase and the threat actor.}
    \label{fig:tsriskassessment}
\end{figure*}

\begin{figure*}[h!]
    \centering
    \includegraphics[trim={1.8cm 11cm 1.8cm 0},clip, width=0.99\textwidth]{sections/figures/attackmapping.pdf}
    \caption{Mapping the capabilities required for implementing the attack on a scale between 0 and 1 (where 0 represents a capability that is not required, and 1 represents a necessary capability) as well as the potential impact of the attack.}
    \label{fig:attackmapping}
\end{figure*}

\begin{figure*}[h!]
    \centering
    \includegraphics[trim={1.8cm 6.5cm 1.8cm 0},clip, width=0.99\textwidth]{sections/figures/tsriskanalysis.pdf}
    \caption{Presenting the derived risk scores for each attack technique within the selected use case.
    The risk is the multiplication of the ranked impact, the likelihood of the attack and the effectiveness of the attack.}
    \label{fig:tsriskassessmenttechnique}
\end{figure*}


\begin{figure*}[h!]
    \centering
    \includegraphics[trim={1.8cm 11.5cm 1.8cm 0},clip, width=0.99\textwidth]{sections/figures/attackprioritization.pdf}
    \caption{Presenting the various attacks  sorted according to the computed risk. 
    USing This sorting makes it possible to prioritize which countermeasures should be considered.
.}
    \label{fig:attackprioritization}
\end{figure*}


==> sections/Tables/Attack_Description_Table.tex <==
\setlength\tabcolsep{4.2pt}
\begin{table*}[tb]
\scriptsize
\centering
\hspace*{-0.5cm}
% \rotatebox{90}
%\resizebox{1.18\textwidth}{0.515\textheight}
{\begin{tabular}{|l"m{0.2\textwidth}"m{0.725\textwidth}|}
\Xhline{3\arrayrulewidth}

\makecell{\textbf{Threat} \\ \textbf{Category}} &
\textbf{Attack Family} &
\textbf{Description} \\
\Xhline{3\arrayrulewidth}

% Evasion [T1]
\multirow{3}{*}{\textbf{\shortstack[l]{Evasion}}} 

&
Gradient-based evasion (white-box) &
The adversary manipulates an input sample in such a way that the classification loss is maximized.
The specific manipulation is determined by calculating the gradients of the classification loss with respect to the input sample~\cite{goodfellow2014explaining,kurakin2016adversarial,carlini2017adversarial}. \\ 
\cline{2-3}
&
Query-based evasion (interactive-black box) &
The adversary interactively queries the model and \textit{estimates} the gradients of the classification loss with respect to the input sample, based on the classification results~\cite{chen2017zoo,chen2020hopskipjumpattack} \\ 
\cline{2-3}

& 
Transferability-based evasion (complete black-box) &
Exploits the \textit{transferability} property of ML models~\cite{papernot2016transferability,szegedy2013intriguing,goodfellow2014explaining}, i.e., adversarial examples that affect one model can often affect other models.
To exploit this property, the adversary creates a surrogate model by training a learning algorithm on a reference dataset and generates adversarial examples by executing white-box gradient-based attacks on the surrogate model.
Then, the adversary uses the adversarial examples to attack the target model.\\
\Xhline{3\arrayrulewidth}


% ML model corruption [T2]
\multirow{2}{*}{\makecell{\shortstack[l]{\textbf{Model} \\ \textbf{Corruption}}}} 
&
Gradient-based poisoning (white-box) &
The adversary manipulates a small number of training samples in such a way that the classification loss of some other set of samples targeted by the attacker is maximized.
The specific manipulation is calculated by solving, using gradient-optimization techniques, a bi-level optimization problem~\cite{kravchik2021poisoning,mei2015using,jagielski2018manipulating}.\\
\cline{2-3}

&
Transferability-based poisoning (black-box). & 
Similar to gradient-based poisoning attacks, manipulates a small number of training samples in such a way that the classification loss of some other set of samples targeted by the attacker is maximized. 
However, in contrast to gradient-based poisoning attacks, the gradients are calculated using a surrogate model~\cite{biggio2012poisoning,munoz2017towards,jagielski2018manipulating}\\
\Xhline{3\arrayrulewidth}


% Membership inference [T3]
\multirow{2}{*}{\makecell{\shortstack[l]{\textbf{Membership} \\\textbf{Inference}}}}
&
Gradient-based inference (white-box). &
The adversary calculates the gradients of the loss with respect to all parameters and analyzes the distribution of these gradients on members of the training data, versus non-members \cite{nasr2019comprehensive}.
The rationale behind this attack is the fact that the gradients of training examples are pushed to zero during the training procedure.\\
\cline{2-3}

&
Query-based inference (black-box) &
The adversary utilizes reference data to train multiple shadow models, which  are meant to behave similarly to the target model; note that the adversary knows which record was included in the training dataset of each shadow model.
Then, the adversary trains a supervised machine learning model that can distinguish between members of training data, versus non-members (attack model).
Finally, given a record, the adversary queries the target model and passes the label, along with the returned vector of probabilities, to the attack model for classification~\cite{shokri2017membership,ateniese2015hacking,ganju2018property,song2020information}.\\
\Xhline{3\arrayrulewidth}

% Membership inference [T3]
\multirow{2}{*}{\makecell{\shortstack[l]{\textbf{Data} \\\textbf{Reconstruction}}}}
&
Gradient-based data reconstruction (white-box) &
The adversary reconstructs the model by making use of gradient-based optimization methods.
That is, the adversary tries to find the optimal data for a given class~\cite{fredrikson2015model,lee1994inverse,linden1989inversion,lu1999inverting,jensen1999inversion,mahendran2015understanding}.\\

\cline{2-3}

&
Query-based data reconstruction (black-box) &
The adversary reconstructs the model by training a second model that acts as the inverse of the target model~\cite{yang2019adversarial,dosovitskiy2016inverting,dosovitskiy2016generating,nash2019inverting}.\\
\Xhline{3\arrayrulewidth}

% Model Extraction [T6]
\makecell{\shortstack[l]{\textbf{Model} \\ \textbf{Extraction}}}

&
Query-based model extraction (black-box). &
The adversary tries to reconstruct the model's parameters by querying the model with specific inputs crafted by the adversary~\cite{tramer2016stealing,chandrasekaran2020exploring,juuti2019prada,oh2019towards,papernot2017practical}.\\ 
\Xhline{3\arrayrulewidth}


% Resource Exhaustion [T7]
\multirow{3}{*}{\makecell{\shortstack[l]{\textbf{Resource} \\ \textbf{Exhaustion}}}}

&
Gradient-based resource exhaustion (white-box) &
The adversary searches (using gradient optimization method) for inputs that increase activation values of the model across all of the layers simultaneously.
High activation values prevent hardware optimization and therefore increase latency~\cite{shumailov2020sponge}. \\
\cline{2-3}

&
Query-based resource exhaustion (interactive black-box) &
The adversary searches (using a genetic algorithm) for inputs that increase model's latency.
In contrast to the gradient-based method, this method does not require access to the model's parameters~ \cite{shumailov2020sponge}. \\
\cline{2-3}

&
Transferability-based resource exhaustion (complete black-box) &
In this type of attack, the adversary creates a surrogate model and searches (using a genetic algorithm or gradient-based optimization) for inputs that increase models' latency.\\
\Xhline{3\arrayrulewidth}

\end{tabular}}
\caption{Adversarial machine learning attack families.}
\label{tab:attack_desc}
\end{table*}

==> sections/Tables/Attack_Table_with_Actors.tex <==
\setlength\tabcolsep{4.2pt}
\begin{table*}[tb]
\tiny
\centering
\hspace*{-1.5cm}
% \rotatebox{90}
%\resizebox{1.15\textwidth}{0.42\textheight}
{\begin{tabular}{@{}
|m{0.13\textwidth}"  % Threat Category
m{0.24\textwidth}|  % Attack Technique
m{0.001\textwidth}m{0.001\textwidth}m{0.001\textwidth}m{0.001\textwidth}|  % AKD
m{0.001\textwidth}m{0.001\textwidth}m{0.001\textwidth}m{0.001\textwidth}|  % AKM
m{0.001\textwidth}m{0.001\textwidth}m{0.001\textwidth}m{0.001\textwidth}|  % ACD
m{0.001\textwidth}m{0.001\textwidth}|  % ACM
m{0.001\textwidth}m{0.001\textwidth}m{0.001\textwidth}"  % Impact
% ||m{0.001\textwidth}|  % Help Titles
m{0.001\textwidth}m{0.001\textwidth}m{0.001\textwidth}m{0.001\textwidth}m{0.001\textwidth}|  % SW App Dev
m{0.001\textwidth}m{0.001\textwidth}m{0.001\textwidth}m{0.001\textwidth}m{0.001\textwidth}|  % SW ISX Dev-nonRT
m{0.001\textwidth}m{0.001\textwidth}m{0.001\textwidth}m{0.001\textwidth}m{0.001\textwidth}|  % SW ISX Dev-nRT
m{0.001\textwidth}m{0.001\textwidth}m{0.001\textwidth}m{0.001\textwidth}m{0.001\textwidth}|  % SW ISX Dev-CUDU
c|  % Contatiner SW ISX Prov
c|  % HW ISX Prov
c|  % UE
% @{}  % Last col space=0
}
\Xhline{3\arrayrulewidth}

\multirow{5}{*}{\makecell{\textbf{Attack}\\\textbf{Family}}} &
\multirow{5}{*}{\textbf{Attack Technique}} &
\multicolumn{17}{c"}{\textbf{Threat Model}} & 
\multicolumn{23}{c|}{\textbf{Threat Actor}} \\
\cline{3-42} 

& & 
\multicolumn{8}{c|}{Knowledge} &
\multicolumn{6}{c|}{Access} & 
\multicolumn{3}{c"}{Impact} & 
\multicolumn{5}{c|}{\textbf{\textit{A1}} } &  % O-RAN SW-App Dev
\multicolumn{15}{c|}{\textbf{\textit{A2}} } &  % O-RAN SW-ISX Dev
\textbf{\textit{A3}} &  % Containerization SW-ISX Prov
\textbf{\textit{A4}} &  % HW-IDX Prov
\textbf{\textit{A5}} \\  % UE
\cline{3-42} 


& & 
\multicolumn{4}{c|}{AKD} &  % Knowledge
\multicolumn{4}{c|}{AKM} &  % Knowledge
\multicolumn{4}{c|}{ACD} &  % Access
\multicolumn{2}{c|}{ACM} &  % Access
\multicolumn{3}{c"}{} &  % Impact
\rotatebox{90}{Data Collection} &  % SW-App Dev
\rotatebox{90}{Data Host} &  % SW-App Dev
\rotatebox{90}{Training Host} &  % SW-App Dev
\rotatebox{90}{Serving Host} &  % SW-App Dev
\rotatebox{90}{ML App} &  % SW-App Dev
\multicolumn{5}{c|}{\makecell{Non-RT\\RIC}} &  % SW-ISX Dev
\multicolumn{5}{c|}{\makecell{Near-RT\\RIC}} &  % SW-ISX Dev
\multicolumn{5}{c|}{\makecell{O-CU / \\O-DU}} &  % SW-ISX Dev
\rotatebox{90}{\makecell{All}} &  % C14n SW-ISX Prov
\rotatebox{90}{\makecell{All}} &  % HW-ISX Prov
\rotatebox{90}{\makecell{All}} \\  % UE
\cline{3-42} 

& & 
% Data Knowledge
\rotatebox{90}{Training Data Knowledge} & 
\rotatebox{90}{Features Data Knowledge} & 
\rotatebox{90}{Raw Data Knowledge} & 
\rotatebox{90}{Data Property Knowledge} &

% Model Knowledge
\rotatebox{90}{Model Knowledge} &
\rotatebox{90}{Hyperparameter Knowledge} &
\rotatebox{90}{Algorithm Knowledge} &
\rotatebox{90}{Task Knowledge} &

% Data Access
\rotatebox{90}{Training Data Access} &
\rotatebox{90}{Features Data Access} &
\rotatebox{90}{Raw Data Access} &
\rotatebox{90}{Sensor Data Access} &

% Model Access
\rotatebox{90}{Score-Based Query Access} &
\rotatebox{90}{Decision-Based Query Access} &

% Impact
\rotatebox{90}{Tampering} &
\rotatebox{90}{Denial of Service} &
\rotatebox{90}{Information Disclosure} & 

% O-RAN SW-App Dev (DS)
\multicolumn{5}{c|}{\rotatebox{90}{\makecell{All}}} & 

% O-RAN SW-ISX Dev (DS)
\rotatebox{90}{\textit{DS 1}} & \rotatebox{90}{\textit{DS 2}} & \rotatebox{90}{\textit{DS 3}} & \rotatebox{90}{\textit{DS 4}} & \rotatebox{90}{\textit{DS 5}} &  %  Non-RT RIC
\rotatebox{90}{\textit{DS 1}} & \rotatebox{90}{\textit{DS 2}} & \rotatebox{90}{\textit{DS 3}} & \rotatebox{90}{\textit{DS 4}} & \rotatebox{90}{\textit{DS 5}} &  %  Near-RT RIC
\rotatebox{90}{\textit{DS 1}} & \rotatebox{90}{\textit{DS 2}} & \rotatebox{90}{\textit{DS 3}} & \rotatebox{90}{\textit{DS 4}} & \rotatebox{90}{\textit{DS 5}} &  %  O-CU/O-DU
\rotatebox{90}{All} &  % C14n SW-IDX Prov
\rotatebox{90}{All} &  % HW-IDX Prov
\rotatebox{90}{All} \\  % UE
\Xhline{3\arrayrulewidth}


% Evasion
	
\rowcolor{Grey}
\multicolumn{42}{|c|}{\textbf{Threat Category:} Evasion}\\ 
\multirow{2}{*}{\textbf{\shortstack[l]{Gradient-based \\evasion attacks}}} 
&
training data and hyperparameter knowledge &
$\bullet$ & $\circ$ & $\circ$  & $\circ$ &  % AKD
$\circ$ & $\bullet$ & $\circ$ & $\circ$ &  % AKM
$\circ$ & $\circ$ & $\circ$ & $\odot$ &  % ACD
$\circ$ & $\odot$ &  % ACM
$\bullet$ & $\circ$ & $\circ$ &  % AG
$\circ$ & $\circ$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-App Dev
$\bullet$ & $\bullet$ & $\circ$ & $\bullet$ & $\circ$ &  % O-RAN SW-ISX Dev - Non
$\circ$ & $\bullet$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-ISX Dev - Near
$\circ$ & $\circ$ & $\circ$ & $\circ$ & $\bullet$ &  % O-RAN SW-ISX Dev - CUDU
$\bullet$ &  % C14n SW-ISX Prov
$\bullet$ &  % HW-ISX Prov
$\circ$ \\  % UE

&
model knowledge &
$\circ$ & $\circ$ & $\circ$  & $\circ$ &  % AKD
$\bullet$ & $\circ$ & $\circ$ & $\circ$ &  % AKM
$\circ$ & $\circ$ & $\circ$ & $\odot$ &  % ACD
$\circ$ & $\odot$ &  % ACM
$\bullet$ & $\circ$ & $\circ$ &  % AG
$\circ$ & $\circ$ & $\bullet$ & $\bullet$ & $\circ$ &  % O-RAN SW-App Dev
$\bullet$ & $\bullet$ & $\circ$ & $\bullet$ & $\circ$ &  % O-RAN SW-ISX Dev - Non
$\circ$ & $\bullet$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-ISX Dev - Near
$\circ$ & $\circ$ & $\circ$ & $\bullet$ & $\bullet$ &  % O-RAN SW-ISX Dev - CUDU
$\bullet$ &  % C14n SW-ISX Prov
$\bullet$ &  % HW-ISX Prov
$\circ$ \\  % UE

\hline

\multirow{2}{*}{\textbf{\shortstack[l]{Query-based \\evasion attacks}}} 
&
model's score (i.e., vector of probabilities) &
$\circ$ & $\circ$ & $\circ$  & $\circ$  &  % AKD
$\circ$ & $\circ$ & $\circ$ & $\bullet$ &  % AKM
$\circ$ & $\circ$ & $\circ$ & $\bullet$ &  % ACD
$\bullet$ & $\circ$ &  % ACM
$\bullet$ & $\circ$ & $\circ$ &  % AG
$\circ$ & $\circ$ & $\bullet$ & $\bullet$ & $\bullet$ &  % O-RAN SW-App Dev
$\bullet$ & $\bullet$ & $\circ$ & $\bullet$ & $\circ$ &  % O-RAN SW-ISX Dev - Non
$\bullet$ & $\bullet$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-ISX Dev - Near
$\circ$ & $\circ$ & $\circ$ & $\bullet$ & $\bullet$ &  % O-RAN SW-ISX Dev - CUDU
$\bullet$ &  % C14n SW-ISX Prov
$\bullet$ &  % HW-ISX Prov
$\circ$ \\  % UE

&
model's decision &
$\circ$ & $\circ$ & $\circ$  & $\circ$  &  % AKD
$\circ$ & $\circ$ & $\circ$ & $\bullet$ &  % AKM
$\circ$ & $\circ$ & $\circ$ & $\bullet$ &  % ACD
$\circ$ & $\bullet$ &  % ACM
$\bullet$ & $\circ$ & $\circ$ &  % AG
$\circ$ & $\circ$ & $\bullet$ & $\bullet$ & $\bullet$ &  % O-RAN SW-App Dev
$\bullet$ & $\bullet$ & $\circ$ & $\bullet$ & $\circ$ &  % O-RAN SW-ISX Dev - Non
$\bullet$ & $\bullet$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-ISX Dev - Near
$\circ$ & $\circ$ & $\circ$ & $\bullet$ & $\bullet$ &  % O-RAN SW-ISX Dev - CUDU
$\bullet$ &  % C14n SW-ISX Prov
$\bullet$ &  % HW-ISX Prov
$\bullet$ \\  % UE
\hline

\multirow{12}{*}{\textbf{\shortstack[l]{Transferability-based\\evasion attacks}}} 
&
training data and hyperparameter knowledge &
$\bullet$ & $\circ$ & $\circ$  & $\circ$  &  % AKD
$\circ$ & $\bullet$ & $\circ$ & $\circ$ &  % AKM
$\circ$ & $\circ$ & $\circ$ & $\odot$ &  % ACD
$\circ$ & $\odot$ &  % ACM
$\bullet$ & $\circ$ & $\circ$ &  % AG
$\circ$ & $\circ$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-App Dev
$\bullet$ & $\bullet$ & $\circ$ & $\bullet$ & $\circ$ &  % O-RAN SW-ISX Dev - Non
$\circ$ & $\bullet$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-ISX Dev - Near
$\circ$ & $\circ$ & $\circ$ & $\bullet$ & $\bullet$ &  % O-RAN SW-ISX Dev - CUDU
$\bullet$ &  % C14n SW-ISX Prov
$\bullet$ &  % HW-ISX Prov
$\circ$ \\  % UE

&
features data and hyperparameter knowledge &
$\circ$ & $\bullet$ & $\circ$  & $\circ$  &  % AKD
$\circ$ & $\bullet$ & $\circ$ & $\circ$ &  % AKM
$\circ$ & $\circ$ & $\circ$ & $\odot$ &  % ACD
$\circ$ & $\odot$ &  % ACM
$\bullet$ & $\circ$ & $\circ$ &  % AG
$\circ$ & $\circ$ & $\bullet$ & $\bullet$ & $\circ$ &  % O-RAN SW-App Dev
$\bullet$ & $\bullet$ & $\circ$ & $\bullet$ & $\circ$ &  % O-RAN SW-ISX Dev - Non
$\circ$ & $\bullet$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-ISX Dev - Near
$\circ$ & $\circ$ & $\circ$ & $\bullet$ & $\bullet$ &  % O-RAN SW-ISX Dev - CUDU
$\bullet$ &  % C14n SW-ISX Prov
$\bullet$ &  % HW-ISX Prov
$\circ$ \\  % UE

&
raw data and hyperparameter knowledge &
$\circ$ & $\circ$ & $\bullet$  & $\circ$  &  % AKD
$\circ$ & $\bullet$ & $\circ$ & $\circ$ &  % AKM
$\circ$ & $\circ$ & $\circ$ & $\odot$ &  % ACD
$\circ$ & $\odot$ &  % ACM
$\bullet$ & $\circ$ & $\circ$ &  % AG
$\circ$ & $\circ$ & $\bullet$ & $\bullet$ & $\circ$ &  % O-RAN SW-App Dev
$\bullet$ & $\bullet$ & $\circ$ & $\bullet$ & $\circ$ &  % O-RAN SW-ISX Dev - Non
$\circ$ & $\bullet$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-ISX Dev - Near
$\circ$ & $\circ$ & $\circ$ & $\bullet$ & $\bullet$ &  % O-RAN SW-ISX Dev - CUDU
$\bullet$ &  % C14n SW-ISX Prov
$\bullet$ &  % HW-ISX Prov
$\circ$ \\  % UE

& 
data property and hyperparameter knowledge &
$\circ$ & $\circ$ & $\circ$  & $\bullet$  &  % AKD
$\circ$ & $\bullet$ & $\circ$ & $\circ$ &  % AKM
$\circ$ & $\circ$ & $\circ$ & $\odot$ &  % ACD
$\circ$ & $\odot$ &  % ACM
$\bullet$ & $\circ$ & $\circ$ &  % AG
$\circ$ & $\circ$ & $\bullet$ & $\bullet$ & $\circ$ &  % O-RAN SW-App Dev
$\bullet$ & $\bullet$ & $\circ$ & $\bullet$ & $\circ$ &  % O-RAN SW-ISX Dev - Non
$\circ$ & $\bullet$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-ISX Dev - Near
$\circ$ & $\circ$ & $\circ$ & $\bullet$ & $\bullet$ &  % O-RAN SW-ISX Dev - CUDU
$\bullet$ &  % C14n SW-ISX Prov
$\bullet$ &  % HW-ISX Prov
$\circ$ \\  % UE

&
training data and algorithm knowledge &
$\bullet$ & $\circ$ & $\circ$  & $\circ$  &  % AKD
$\circ$ & $\circ$ & $\bullet$ & $\circ$ &  % AKM
$\circ$ & $\circ$ & $\circ$ & $\odot$ &  % ACD
$\circ$ & $\odot$ &  % ACM
$\bullet$ & $\circ$ & $\circ$ &  % AG
$\circ$ & $\circ$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-App Dev
$\bullet$ & $\bullet$ & $\circ$ & $\bullet$ & $\circ$ &  % O-RAN SW-ISX Dev - Non
$\circ$ & $\bullet$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-ISX Dev - Near
$\circ$ & $\circ$ & $\circ$ & $\bullet$ & $\bullet$ &  % O-RAN SW-ISX Dev - CUDU
$\bullet$ &  % C14n SW-ISX Prov
$\bullet$ &  % HW-ISX Prov
$\circ$ \\  % UE

&
features data and algorithm knowledge &
$\circ$ & $\bullet$ & $\circ$  & $\circ$  &  % AKD
$\circ$ & $\circ$ & $\bullet$ & $\circ$ &  % AKM
$\circ$ & $\circ$ & $\circ$ & $\odot$ &  % ACD
$\circ$ & $\odot$ &  % ACM
$\bullet$ & $\circ$ & $\circ$ &  % AG
$\circ$ & $\circ$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-App Dev
$\bullet$ & $\bullet$ & $\circ$ & $\bullet$ & $\circ$ &  % O-RAN SW-ISX Dev - Non
$\circ$ & $\bullet$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-ISX Dev - Near
$\circ$ & $\circ$ & $\circ$ & $\bullet$ & $\bullet$ &  % O-RAN SW-ISX Dev - CUDU
$\bullet$ &  % C14n SW-ISX Prov
$\bullet$ &  % HW-ISX Prov
$\circ$ \\  % UE

&
raw data and algorithm knowledge &
$\circ$ & $\circ$ & $\bullet$  & $\circ$  &  % AKD
$\circ$ & $\circ$ & $\bullet$ & $\circ$ &  % AKM
$\circ$ & $\circ$ & $\circ$ & $\odot$ &  % ACD
$\circ$ & $\odot$ &  % ACM
$\bullet$ & $\circ$ & $\circ$ &  % AG
$\circ$ & $\circ$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-App Dev
$\bullet$ & $\bullet$ & $\circ$ & $\bullet$ & $\circ$ &  % O-RAN SW-ISX Dev - Non
$\circ$ & $\bullet$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-ISX Dev - Near
$\circ$ & $\circ$ & $\circ$ & $\bullet$ & $\bullet$ &  % O-RAN SW-ISX Dev - CUDU
$\bullet$ &  % C14n SW-ISX Prov
$\bullet$ &  % HW-ISX Prov
$\circ$ \\  % UE

&
data property and algorithm knowledge &
$\circ$ & $\circ$ & $\circ$  & $\bullet$  &  % AKD
$\circ$ & $\circ$ & $\bullet$ & $\circ$ &  % AKM
$\circ$ & $\circ$ & $\circ$ & $\odot$ &  % ACD
$\circ$ & $\odot$ &  % ACM
$\bullet$ & $\circ$ & $\circ$ &  % AG
$\circ$ & $\circ$ & $\bullet$ & $\bullet$ & $\circ$ &  % O-RAN SW-App Dev
$\bullet$ & $\bullet$ & $\circ$ & $\bullet$ & $\circ$ &  % O-RAN SW-ISX Dev - Non
$\circ$ & $\bullet$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-ISX Dev - Near
$\circ$ & $\circ$ & $\circ$ & $\bullet$ & $\bullet$ &  % O-RAN SW-ISX Dev - CUDU
$\bullet$ &  % C14n SW-ISX Prov
$\bullet$ &  % HW-ISX Prov
$\circ$ \\  % UE

&
training data and task knowledge &
$\bullet$ & $\circ$ & $\circ$  & $\circ$  &  % AKD
$\circ$ & $\circ$ & $\circ$ & $\bullet$ &  % AKM
$\circ$ & $\circ$ & $\circ$ & $\odot$ &  % ACD
$\circ$ & $\odot$ &  % ACM
$\bullet$ & $\circ$ & $\circ$ &  % AG
$\circ$ & $\circ$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-App Dev
$\bullet$ & $\bullet$ & $\circ$ & $\bullet$ & $\circ$ &  % O-RAN SW-ISX Dev - Non
$\bullet$ & $\bullet$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-ISX Dev - Near
$\circ$ & $\circ$ & $\circ$ & $\bullet$ & $\bullet$ &  % O-RAN SW-ISX Dev - CUDU
$\bullet$ &  % C14n SW-ISX Prov
$\bullet$ &  % HW-ISX Prov
$\circ$ \\  % UE

&
features data and task knowledge &
$\circ$ & $\bullet$ & $\circ$  & $\circ$  &  % AKD
$\circ$ & $\circ$ & $\circ$ & $\bullet$ &  % AKM
$\circ$ & $\circ$ & $\circ$ & $\odot$ &  % ACD
$\circ$ & $\odot$ &  % ACM
$\bullet$ & $\circ$ & $\circ$ &  % AG
$\circ$ & $\bullet$ & $\bullet$ & $\bullet$ & $\circ$ &  % O-RAN SW-App Dev
$\bullet$ & $\bullet$ & $\circ$ & $\bullet$ & $\circ$ &  % O-RAN SW-ISX Dev - Non
$\bullet$ & $\bullet$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-ISX Dev - Near
$\circ$ & $\circ$ & $\circ$ & $\bullet$ & $\bullet$ &  % O-RAN SW-ISX Dev - CUDU
$\bullet$ &  % C14n SW-ISX Prov
$\bullet$ &  % HW-ISX Prov
$\circ$ \\  % UE

&
raw data and task knowledge &
$\circ$ & $\circ$ & $\bullet$  & $\circ$  &  % AKD
$\circ$ & $\circ$ & $\circ$ & $\bullet$ &  % AKM
$\circ$ & $\circ$ & $\circ$ & $\odot$ &  % ACD
$\circ$ & $\odot$ &  % ACM
$\bullet$ & $\circ$ & $\circ$ &  % AG
$\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ &  % O-RAN SW-App Dev
$\bullet$ & $\bullet$ & $\circ$ & $\bullet$ & $\circ$ &  % O-RAN SW-ISX Dev - Non
$\bullet$ & $\bullet$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-ISX Dev - Near
$\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ &  % O-RAN SW-ISX Dev - CUDU
$\bullet$ &  % C14n SW-ISX Prov
$\bullet$ &  % HW-ISX Prov
$\circ$ \\  % UE
&
data property and task knowledge &
$\circ$ & $\circ$ & $\circ$  & $\bullet$  &  % AKD
$\circ$ & $\circ$ & $\circ$ & $\bullet$ &  % AKM
$\circ$ & $\circ$ & $\circ$ & $\odot$ &  % ACD
$\circ$ & $\odot$ &  % ACM
$\bullet$ & $\circ$ & $\circ$ &  % AG
$\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ &  % O-RAN SW-App Dev
$\bullet$ & $\bullet$ & $\circ$ & $\bullet$ & $\circ$ &  % O-RAN SW-ISX Dev - Non
$\bullet$ & $\bullet$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-ISX Dev - Near
$\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ &  % O-RAN SW-ISX Dev - CUDU
$\bullet$ &  % C14n SW-ISX Prov
$\bullet$ &  % HW-ISX Prov
$\circ$ \\  % UE

\Xhline{3\arrayrulewidth}


\rowcolor{Grey}
\multicolumn{42}{|c|}{\textbf{Threat Category:} Model Corruption}\\ 

\textbf{\shortstack[l]{Gradient-based\\poisoning attacks}}
&
model knowledge &
$\circ$ & $\circ$ & $\circ$  & $\circ$  &  % AKD
$\bullet$ & $\circ$ & $\circ$ & $\circ$ &  % AKM
$\bullet$ & $\circ$ & $\circ$ & $\circ$ &  % ACD
$\circ$ & $\circ$ &  % ACM
$\bullet$ & $\bullet$ & $\circ$ &  % AG
$\circ$ & $\circ$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-App Dev
$\bullet$ & $\bullet$ & $\circ$ & $\bullet$ & $\circ$ &  % O-RAN SW-ISX Dev - Non
$\circ$ & $\bullet$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-ISX Dev - Near
$\circ$ & $\circ$ & $\circ$ & $\bullet$ & $\bullet$ &  % O-RAN SW-ISX Dev - CUDU
$\bullet$ &  % C14n SW-ISX Prov
$\bullet$ &  % HW-ISX Prov
$\circ$ \\  \hline

\multirow{12}{*}{\textbf{\shortstack[l]{Transferability-based \\poisoning attacks}}} 
&
training data and hyperparameter knowledge &
$\bullet$ & $\circ$ & $\circ$  & $\circ$  &  % AKD
$\circ$ & $\bullet$ & $\circ$ & $\circ$ &  % AKM
$\bullet$ & $\circ$ & $\circ$ & $\circ$ &  % ACD
$\circ$ & $\circ$ &  % ACM
$\bullet$ & $\bullet$ & $\circ$ &  % AG
$\circ$ & $\circ$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-App Dev
$\bullet$ & $\bullet$ & $\circ$ & $\bullet$ & $\circ$ &  % O-RAN SW-ISX Dev - Non
$\circ$ & $\bullet$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-ISX Dev - Near
$\circ$ & $\circ$ & $\circ$ & $\bullet$ & $\bullet$ &  % O-RAN SW-ISX Dev - CUDU
$\bullet$ &  % C14n SW-ISX Prov
$\bullet$ &  % HW-ISX Prov
$\circ$ \\  % UE


&
features data and hyperparameter knowledge &
$\circ$ & $\bullet$ & $\circ$  & $\circ$  &  % AKD
$\circ$ & $\bullet$ & $\circ$ & $\circ$ &  % AKM
$\bullet$ & $\circ$ & $\circ$ & $\circ$ &  % ACD
$\circ$ & $\circ$ &  % ACM
$\bullet$ & $\bullet$ & $\circ$ &  % AG
$\circ$ & $\circ$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-App Dev
$\bullet$ & $\bullet$ & $\circ$ & $\bullet$ & $\circ$ &  % O-RAN SW-ISX Dev - Non
$\circ$ & $\bullet$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-ISX Dev - Near
$\circ$ & $\circ$ & $\circ$ & $\bullet$ & $\bullet$ &  % O-RAN SW-ISX Dev - CUDU
$\bullet$ &  % C14n SW-ISX Prov
$\bullet$ &  % HW-ISX Prov
$\circ$ \\  % UE


&
raw data and hyperparameter knowledge &
$\circ$ & $\circ$ & $\bullet$  & $\circ$  &  % AKD
$\circ$ & $\bullet$ & $\circ$ & $\circ$ &  % AKM
$\bullet$ & $\circ$ & $\circ$ & $\circ$ &  % ACD
$\circ$ & $\circ$ &  % ACM
$\bullet$ & $\bullet$ & $\circ$ &  % AG
$\circ$ & $\circ$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-App Dev
$\bullet$ & $\bullet$ & $\circ$ & $\bullet$ & $\circ$ &  % O-RAN SW-ISX Dev - Non
$\circ$ & $\bullet$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-ISX Dev - Near
$\circ$ & $\circ$ & $\circ$ & $\bullet$ & $\bullet$ &  % O-RAN SW-ISX Dev - CUDU
$\bullet$ &  % C14n SW-ISX Prov
$\bullet$ &  % HW-ISX Prov
$\circ$ \\  % UE

&
data property and hyperparameter knowledge &
$\circ$ & $\circ$ & $\circ$  & $\bullet$  &  % AKD
$\circ$ & $\bullet$ & $\circ$ & $\circ$ &  % AKM
$\bullet$ & $\circ$ & $\circ$ & $\circ$ &  % ACD
$\circ$ & $\circ$ &  % ACM
$\bullet$ & $\bullet$ & $\circ$ &  % AG
$\circ$ & $\circ$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-App Dev
$\bullet$ & $\bullet$ & $\circ$ & $\bullet$ & $\circ$ &  % O-RAN SW-ISX Dev - Non
$\circ$ & $\bullet$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-ISX Dev - Near
$\circ$ & $\circ$ & $\circ$ & $\bullet$ & $\bullet$ &  % O-RAN SW-ISX Dev - CUDU
$\bullet$ &  % C14n SW-ISX Prov
$\bullet$ &  % HW-ISX Prov
$\circ$ \\  % UE

&
training data and algorithm knowledge &
$\bullet$ & $\circ$ & $\circ$  & $\circ$  &  % AKD
$\circ$ & $\circ$ & $\bullet$ & $\circ$ &  % AKM
$\bullet$ & $\circ$ & $\circ$ & $\circ$ &  % ACD
$\circ$ & $\circ$ &  % ACM
$\bullet$ & $\bullet$ & $\circ$ &  % AG
$\circ$ & $\circ$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-App Dev
$\bullet$ & $\bullet$ & $\circ$ & $\bullet$ & $\circ$ &  % O-RAN SW-ISX Dev - Non
$\circ$ & $\bullet$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-ISX Dev - Near
$\circ$ & $\circ$ & $\circ$ & $\bullet$ & $\bullet$ &  % O-RAN SW-ISX Dev - CUDU
$\bullet$ &  % C14n SW-ISX Prov
$\bullet$ &  % HW-ISX Prov
$\circ$ \\  % UE


&
features data and algorithm knowledge &
$\circ$ & $\bullet$ & $\circ$  & $\circ$  &  % AKD
$\circ$ & $\circ$ & $\bullet$ & $\circ$ &  % AKM
$\bullet$ & $\circ$ & $\circ$ & $\circ$ &  % ACD
$\circ$ & $\circ$ &  % ACM
$\bullet$ & $\bullet$ & $\circ$ &  % AG
$\circ$ & $\circ$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-App Dev
$\bullet$ & $\bullet$ & $\circ$ & $\bullet$ & $\circ$ &  % O-RAN SW-ISX Dev - Non
$\circ$ & $\bullet$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-ISX Dev - Near
$\circ$ & $\circ$ & $\circ$ & $\bullet$ & $\bullet$ &  % O-RAN SW-ISX Dev - CUDU
$\bullet$ &  % C14n SW-ISX Prov
$\bullet$ &  % HW-ISX Prov
$\circ$ \\  % UE

&
raw data and algorithm knowledge &
$\circ$ & $\circ$ & $\bullet$  & $\circ$  &  % AKD
$\circ$ & $\circ$ & $\bullet$ & $\circ$ &  % AKM
$\bullet$ & $\circ$ & $\circ$ & $\circ$ &  % ACD
$\circ$ & $\circ$ &  % ACM
$\bullet$ & $\bullet$ & $\circ$ &  % AG
$\circ$ & $\circ$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-App Dev
$\bullet$ & $\bullet$ & $\circ$ & $\bullet$ & $\circ$ &  % O-RAN SW-ISX Dev - Non
$\circ$ & $\bullet$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-ISX Dev - Near
$\circ$ & $\circ$ & $\circ$ & $\bullet$ & $\bullet$ &  % O-RAN SW-ISX Dev - CUDU
$\bullet$ &  % C14n SW-ISX Prov
$\bullet$ &  % HW-ISX Prov
$\circ$ \\  % UE

&
data property and algorithm knowledge &
$\circ$ & $\circ$ & $\circ$  & $\bullet$  &  % AKD
$\circ$ & $\circ$ & $\bullet$ & $\circ$ &  % AKM
$\bullet$ & $\circ$ & $\circ$ & $\circ$ &  % ACD
$\circ$ & $\circ$ &  % ACM
$\bullet$ & $\bullet$ & $\circ$ &  % AG
$\circ$ & $\circ$ & $\bullet$ & $\bullet$ & $\circ$ &  % O-RAN SW-App Dev
$\bullet$ & $\bullet$ & $\circ$ & $\bullet$ & $\circ$ &  % O-RAN SW-ISX Dev - Non
$\circ$ & $\bullet$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-ISX Dev - Near
$\circ$ & $\circ$ & $\circ$ & $\bullet$ & $\bullet$ &  % O-RAN SW-ISX Dev - CUDU
$\bullet$ &  % C14n SW-ISX Prov
$\bullet$ &  % HW-ISX Prov
$\circ$ \\  % UE

&
training data and task knowledge &
$\bullet$ & $\circ$ & $\circ$  & $\circ$  &  % AKD
$\circ$ & $\circ$ & $\circ$ & $\bullet$ &  % AKM
$\bullet$ & $\circ$ & $\circ$ & $\circ$ &  % ACD
$\circ$ & $\circ$ &  % ACM
$\bullet$ & $\bullet$ & $\circ$ &  % AG
$\circ$ & $\bullet$ & $\bullet$ & $\bullet$ & $\circ$ &  % O-RAN SW-App Dev
$\bullet$ & $\bullet$ & $\circ$ & $\bullet$ & $\circ$ &  % O-RAN SW-ISX Dev - Non
$\bullet$ & $\bullet$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-ISX Dev - Near
$\circ$ & $\circ$ & $\circ$ & $\bullet$ & $\bullet$ &  % O-RAN SW-ISX Dev - CUDU
$\bullet$ &  % C14n SW-ISX Prov
$\bullet$ &  % HW-ISX Prov
$\circ$ \\  % UE

&
features data and task knowledge &
$\circ$ & $\bullet$ & $\circ$  & $\circ$  &  % AKD
$\circ$ & $\circ$ & $\circ$ & $\bullet$ &  % AKM
$\bullet$ & $\circ$ & $\circ$ & $\circ$ &  % ACD
$\circ$ & $\circ$ &  % ACM
$\bullet$ & $\bullet$ & $\circ$ &  % AG
$\circ$ & $\bullet$ & $\bullet$ & $\bullet$ & $\circ$ &  % O-RAN SW-App Dev
$\bullet$ & $\bullet$ & $\circ$ & $\bullet$ & $\circ$ &  % O-RAN SW-ISX Dev - Non
$\bullet$ & $\bullet$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-ISX Dev - Near
$\circ$ & $\circ$ & $\circ$ & $\bullet$ & $\bullet$ &  % O-RAN SW-ISX Dev - CUDU
$\bullet$ &  % C14n SW-ISX Prov
$\bullet$ &  % HW-ISX Prov
$\circ$ \\  % UE

&
raw data and task knowledge &
$\circ$ & $\circ$ & $\bullet$  & $\circ$  &  % AKD
$\circ$ & $\circ$ & $\circ$ & $\bullet$ &  % AKM
$\bullet$ & $\circ$ & $\circ$ & $\circ$ &  % ACD
$\circ$ & $\circ$ &  % ACM
$\bullet$ & $\bullet$ & $\circ$ &  % AG
$\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ & $\circ$ &  % O-RAN SW-App Dev
$\bullet$ & $\bullet$ & $\circ$ & $\bullet$ & $\circ$ &  % O-RAN SW-ISX Dev - Non
$\bullet$ & $\bullet$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-ISX Dev - Near
$\odot$ & $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ &  % O-RAN SW-ISX Dev - CUDU
$\bullet$ &  % C14n SW-ISX Prov
$\bullet$ &  % HW-ISX Prov
$\circ$ \\  % UE

&
data property and task knowledge &
$\circ$ & $\circ$ & $\circ$  & $\bullet$  &  % AKD
$\circ$ & $\circ$ & $\circ$ & $\bullet$ &  % AKM
$\bullet$ & $\circ$ & $\circ$ & $\circ$ &  % ACD
$\circ$ & $\circ$ &  % ACM
$\bullet$ & $\bullet$ & $\circ$ &  % AG
$\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ & $\circ$ &  % O-RAN SW-App Dev
$\bullet$ & $\bullet$ & $\circ$ & $\bullet$ & $\circ$ &  % O-RAN SW-ISX Dev - Non
$\bullet$ & $\bullet$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-ISX Dev - Near
$\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ &  % O-RAN SW-ISX Dev - CUDU
$\bullet$ &  % C14n SW-ISX Prov
$\bullet$ &  % HW-ISX Prov
$\circ$ \\  % UE
\Xhline{3\arrayrulewidth}


% Inference and Reconstruction
\rowcolor{Grey}
\multicolumn{42}{|c|}{\textbf{Threat Category:} Membership Inference}\\ 
\textbf{\shortstack[l]{Gradient-based\\inference attacks}}
&
model knowledge (e.g., when using public models) &
$\circ$ & $\circ$ & $\circ$  & $\circ$  &  % AKD
$\bullet$ & $\circ$ & $\circ$ & $\circ$ &  % AKM
$\circ$ & $\circ$ & $\circ$ & $\circ$ &  % ACD
$\circ$ & $\circ$ &  % ACM
$\circ$ & $\circ$ & $\bullet$ &  % AG
$\circ$ & $\circ$ & $\bullet$ & $\bullet$ & $\circ$ &  % O-RAN SW-App Dev
$\bullet$ & $\bullet$ & $\circ$ & $\bullet$ & $\circ$ &  % O-RAN SW-ISX Dev - Non
$\circ$ & $\bullet$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-ISX Dev - Near
$\circ$ & $\circ$ & $\circ$ & $\bullet$ & $\bullet$ &  % O-RAN SW-ISX Dev - CUDU
$\bullet$ &  % C14n SW-ISX Prov
$\bullet$ &  % HW-ISX Prov
$\circ$ \\  % UE
\hline

\textbf{\shortstack[l]{Query-based\\inference attacks}} 
&
query access and data property knowledge&
$\circ$ & $\circ$ & $\circ$  & $\bullet$  &  % AKD
$\circ$ &  $\circ$ & $\circ$ & $\bullet$ &  % AKM
$\circ$ & $\circ$ & $\circ$ & $\bullet$ &  % ACD
$\bullet$ & $\circ$ &  % ACM
$\circ$ & $\circ$ & $\bullet$ &  % AG
$\circ$ & $\circ$ & $\bullet$ & $\bullet$ & $\bullet$ &  % O-RAN SW-App Dev
$\bullet$ & $\bullet$ & $\circ$ & $\bullet$ & $\circ$ &  % O-RAN SW-ISX Dev - Non
$\bullet$ & $\bullet$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-ISX Dev - Near
$\circ$ & $\circ$ & $\circ$ & $\bullet$ & $\bullet$ &  % O-RAN SW-ISX Dev - CUDU
$\bullet$ &  % C14n SW-ISX Prov
$\bullet$ &  % HW-ISX Prov
$\circ$ \\  % UE
\Xhline{3\arrayrulewidth}


%  Data Reconstruction
\rowcolor{Grey}
\multicolumn{42}{|c|}{\textbf{Threat Category:} Data Reconstruction}\\ 
\textbf{\shortstack[l]{Gradient-based Data \\Reconstruction attacks}}
& 
model knowledge  &
$\circ$ & $\circ$ & $\circ$  & $\circ$  &  % AKD
$\bullet$ & $\circ$ & $\circ$ & $\circ$ &  % AKM
$\circ$ & $\circ$ & $\circ$ & $\circ$ &  % ACD
$\circ$ & $\circ$ &  % ACM
$\circ$ & $\circ$ & $\bullet$ &  % AG
$\circ$ & $\circ$ & $\bullet$ & $\bullet$ & $\circ$ &  % O-RAN SW-App Dev
$\bullet$ & $\bullet$ & $\circ$ & $\bullet$ & $\circ$ &  % O-RAN SW-ISX Dev - Non
$\circ$ & $\bullet$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-ISX Dev - Near
$\circ$ & $\circ$ & $\circ$ & $\bullet$ & $\bullet$ &  % O-RAN SW-ISX Dev - CUDU
$\bullet$ &  % C14n SW-ISX Prov
$\bullet$ &  % HW-ISX Prov
$\circ$ \\  % UE
\hline
\textbf{\shortstack[l]{Query-based Data\\Reconstruction attacks}} 

&
query access and data property knowledge&
$\circ$ & $\circ$ & $\circ$  & $\bullet$  &  % AKD
$\circ$ &  $\circ$ & $\circ$ & $\bullet$ &  % AKM
$\circ$ & $\circ$ & $\circ$ & $\bullet$ &  % ACD
$\bullet$ & $\circ$ &  % ACM
$\circ$ & $\circ$ & $\bullet$ &  % AG
$\circ$ & $\circ$ & $\bullet$ & $\bullet$ & $\bullet$ &  % O-RAN SW-App Dev
$\bullet$ & $\bullet$ & $\circ$ & $\bullet$ & $\circ$ &  % O-RAN SW-ISX Dev - Non
$\bullet$ & $\bullet$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-ISX Dev - Near
$\circ$ & $\circ$ & $\circ$ & $\bullet$ & $\bullet$ &  % O-RAN SW-ISX Dev - CUDU
$\bullet$ &  % C14n SW-ISX Prov
$\bullet$ &  % HW-ISX Prov
$\circ$ \\  % UE
\Xhline{3\arrayrulewidth}


\rowcolor{Grey}
\multicolumn{42}{|c|}{\textbf{Threat Category:} Model Extraction}\\ 

\multirow{2}{*}{\textbf{\shortstack[l]{Query-based model \\extraction attacks}}} 
&
score-based query access &
$\circ$ & $\circ$ & $\circ$  & $\circ$  &  % AKD
$\circ$ & $\circ$ & $\circ$ & $\circ$ &  % AKM
$\circ$ & $\circ$ & $\circ$ & $\bullet$&  % ACD
$\bullet$ & $\circ$ &  % ACM
$\circ$ & $\circ$ & $\bullet$ &  % AG
$\circ$ & $\circ$ & $\bullet$ & $\bullet$ & $\bullet$ &  % O-RAN SW-App Dev
$\bullet$ & $\bullet$ & $\circ$ & $\bullet$ & $\circ$ &  % O-RAN SW-ISX Dev - Non
$\bullet$ & $\bullet$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-ISX Dev - Near
$\circ$ & $\circ$ & $\circ$ & $\bullet$ & $\bullet$ &  % O-RAN SW-ISX Dev - CUDU
$\bullet$ &  % C14n SW-ISX Prov
$\bullet$ &  % HW-ISX Prov
$\circ$ \\  % UE

&
decision-based query access &
$\circ$ & $\circ$ & $\circ$  & $\circ$  &  % AKD
$\circ$ & $\circ$ & $\circ$ & $\circ$ &  % AKM
$\circ$ & $\circ$ & $\circ$ & $\bullet$&  % ACD
$\circ$ & $\bullet$ &  % ACM
$\circ$ & $\circ$ & $\bullet$ &  % AG
$\circ$ & $\circ$ & $\bullet$ & $\bullet$ & $\bullet$ &  % O-RAN SW-App Dev
$\bullet$ & $\bullet$ & $\circ$ & $\bullet$ & $\circ$ &  % O-RAN SW-ISX Dev - Non
$\bullet$ & $\bullet$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-ISX Dev - Near
$\circ$ & $\circ$ & $\circ$ & $\bullet$ & $\bullet$ &  % O-RAN SW-ISX Dev - CUDU
$\bullet$ &  % C14n SW-ISX Prov
$\bullet$ &  % HW-ISX Prov
$\bullet$ \\  % UE
\Xhline{3\arrayrulewidth}


\rowcolor{Grey}
\multicolumn{42}{|c|}{\textbf{Threat Category:} Resource Exhaustion}\\ 
\multirow{2}{*}{\textbf{\shortstack[l]{Gradient-based resource \\exhaustion attacks}}} 
&
training data and hyperparameter knowledge &
$\bullet$ & $\circ$ & $\circ$  & $\circ$  &  % AKD
$\circ$ & $\bullet$ & $\circ$ & $\circ$ &  % AKM
$\circ$ & $\circ$ & $\circ$ & $\circ$ &  % ACD
$\circ$ & $\odot$ &  % ACM
$\circ$ & $\bullet$ & $\circ$ &  % AG
$\circ$ & $\circ$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-App Dev
$\bullet$ & $\bullet$ & $\circ$ & $\bullet$ & $\circ$ &  % O-RAN SW-ISX Dev - Non
$\circ$ & $\bullet$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-ISX Dev - Near
$\circ$ & $\circ$ & $\circ$ & $\bullet$ & $\bullet$ &  % O-RAN SW-ISX Dev - CUDU
$\bullet$ &  % C14n SW-ISX Prov
$\bullet$ &  % HW-ISX Prov
$\circ$ \\  % UE

&
model's knowledge &
$\circ$ & $\circ$ & $\circ$  & $\circ$  &  % AKD
$\bullet$ & $\circ$ & $\circ$ & $\circ$ &  % AKM
$\circ$ & $\circ$ & $\circ$ & $\circ$ &  % ACD
$\circ$ & $\odot$ &  % ACM
$\circ$ & $\bullet$ & $\circ$ &  % AG
$\circ$ & $\circ$ & $\bullet$ & $\bullet$ & $\circ$ &  % O-RAN SW-App Dev
$\bullet$ & $\bullet$ & $\circ$ & $\bullet$ & $\circ$ &  % O-RAN SW-ISX Dev - Non
$\circ$ & $\bullet$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-ISX Dev - Near
$\circ$ & $\circ$ & $\circ$ & $\bullet$ & $\bullet$ &  % O-RAN SW-ISX Dev - CUDU
$\bullet$ &  % C14n SW-ISX Prov
$\bullet$ &  % HW-ISX Prov
$\circ$ \\  % UE
\hline

\shortstack[l]{\textbf{Query-based resource}\\\textbf{exhaustion attacks}}
&
query based access and model's latency measurements &
$\circ$ & $\circ$ & $\circ$  & $\circ$  &  % AKD
$\circ$ & $\circ$ & $\circ$ & $\bullet$ &  % AKM
$\circ$ & $\circ$ & $\circ$ & $\bullet$ &  % ACD
$\circ$ & $\bullet$ &  % ACM
$\circ$ & $\bullet$ & $\circ$ &  % AG
$\circ$ & $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ &  % O-RAN SW-App Dev
$\bullet$ & $\bullet$ & $\circ$ & $\bullet$ & $\circ$ &  % O-RAN SW-ISX Dev - Non
$\bullet$ & $\bullet$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-ISX Dev - Near
$\circ$ & $\circ$ & $\circ$ & $\bullet$ & $\bullet$ &  % O-RAN SW-ISX Dev - CUDU
$\bullet$ &  % C14n SW-ISX Prov
$\bullet$ &  % HW-ISX Prov
$\bullet$ \\  % UE

\hline

\multirow{12}{*}{\textbf{\shortstack[l]{Transferability-based\\resource exhaustion\\attacks}}} 

&
training data and hyperparameter knowledge &
$\bullet$ & $\circ$ & $\circ$  & $\circ$  &  % AKD
$\circ$ & $\bullet$ & $\circ$ & $\circ$ &  % AKM
$\circ$ & $\circ$ & $\circ$ & $\odot$ &  % ACD
$\circ$ & $\odot$ &  % ACM
$\circ$ & $\bullet$ & $\circ$ &  % AG
$\circ$ & $\circ$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-App Dev
$\bullet$ & $\bullet$ & $\circ$ & $\bullet$ & $\circ$ &  % O-RAN SW-ISX Dev - Non
$\circ$ & $\bullet$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-ISX Dev - Near
$\circ$ & $\circ$ & $\circ$ & $\bullet$ & $\bullet$ &  % O-RAN SW-ISX Dev - CUDU
$\bullet$ &  % C14n SW-ISX Prov
$\bullet$ &  % HW-ISX Prov
$\circ$ \\  % UE

&
features data and hyperparameter knowledge &
$\circ$ & $\bullet$ & $\circ$  & $\circ$  &  % AKD
$\circ$ & $\bullet$ & $\circ$ & $\circ$ &  % AKM
$\circ$ & $\circ$ & $\circ$ & $\odot$ &  % ACD
$\circ$ & $\odot$ &  % ACM
$\circ$ & $\bullet$ & $\circ$ &  % AG
$\circ$ & $\circ$ & $\bullet$ & $\bullet$ & $\circ$ &  % O-RAN SW-App Dev
$\bullet$ & $\bullet$ & $\circ$ & $\bullet$ & $\circ$ &  % O-RAN SW-ISX Dev - Non
$\circ$ & $\bullet$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-ISX Dev - Near
$\circ$ & $\circ$ & $\circ$ & $\bullet$ & $\bullet$ &  % O-RAN SW-ISX Dev - CUDU
$\bullet$ &  % C14n SW-ISX Prov
$\bullet$ &  % HW-ISX Prov
$\circ$ \\  % UE

&
raw data and hyperparameter knowledge &
$\circ$ & $\circ$ & $\bullet$  & $\circ$  &  % AKD
$\circ$ & $\bullet$ & $\circ$ & $\circ$ &  % AKM
$\circ$ & $\circ$ & $\circ$ & $\odot$ &  % ACD
$\circ$ & $\odot$ &  % ACM
$\circ$ & $\bullet$ & $\circ$ &  % AG
$\circ$ & $\circ$ & $\bullet$ & $\bullet$ & $\circ$ &  % O-RAN SW-App Dev
$\bullet$ & $\bullet$ & $\circ$ & $\bullet$ & $\circ$ &  % O-RAN SW-ISX Dev - Non
$\circ$ & $\bullet$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-ISX Dev - Near
$\circ$ & $\circ$ & $\circ$ & $\bullet$ & $\bullet$ &  % O-RAN SW-ISX Dev - CUDU
$\bullet$ &  % C14n SW-ISX Prov
$\bullet$ &  % HW-ISX Prov
$\circ$ \\  % UE

&
data property and hyperparameter knowledge &
$\circ$ & $\circ$ & $\circ$  & $\bullet$  &  % AKD
$\circ$ & $\bullet$ & $\circ$ & $\circ$ &  % AKM
$\circ$ & $\circ$ & $\circ$ & $\odot$ &  % ACD
$\circ$ & $\odot$ &  % ACM
$\circ$ & $\bullet$ & $\circ$ &  % AG
$\circ$ & $\circ$ & $\bullet$ & $\bullet$ & $\circ$ &  % O-RAN SW-App Dev
$\bullet$ & $\bullet$ & $\circ$ & $\bullet$ & $\circ$ &  % O-RAN SW-ISX Dev - Non
$\circ$ & $\bullet$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-ISX Dev - Near
$\circ$ & $\circ$ & $\circ$ & $\bullet$ & $\bullet$ &  % O-RAN SW-ISX Dev - CUDU
$\bullet$ &  % C14n SW-ISX Prov
$\bullet$ &  % HW-ISX Prov
$\circ$ \\  % UE

&
training data and algorithm knowledge &
$\bullet$ & $\circ$ & $\circ$  & $\circ$  &  % AKD
$\circ$ & $\circ$ & $\bullet$ & $\circ$ &  % AKM
$\circ$ & $\circ$ & $\circ$ & $\odot$ &  % ACD
$\circ$ & $\odot$ &  % ACM
$\circ$ & $\bullet$ & $\circ$ &  % AG
$\circ$ & $\circ$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-App Dev
$\bullet$ & $\bullet$ & $\circ$ & $\bullet$ & $\circ$ &  % O-RAN SW-ISX Dev - Non
$\circ$ & $\bullet$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-ISX Dev - Near
$\circ$ & $\circ$ & $\circ$ & $\bullet$ & $\bullet$ &  % O-RAN SW-ISX Dev - CUDU
$\bullet$ &  % C14n SW-ISX Prov
$\bullet$ &  % HW-ISX Prov
$\circ$ \\  % UE

&
features data and algorithm knowledge &
$\circ$ & $\bullet$ & $\circ$  & $\circ$  &  % AKD
$\circ$ & $\circ$ & $\bullet$ & $\circ$ &  % AKM
$\circ$ & $\circ$ & $\circ$ & $\odot$ &  % ACD
$\circ$ & $\odot$ &  % ACM
$\circ$ & $\bullet$ & $\circ$ &  % AG
$\circ$ & $\circ$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-App Dev
$\bullet$ & $\bullet$ & $\circ$ & $\bullet$ & $\circ$ &  % O-RAN SW-ISX Dev - Non
$\circ$ & $\bullet$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-ISX Dev - Near
$\circ$ & $\circ$ & $\circ$ & $\bullet$ & $\bullet$ &  % O-RAN SW-ISX Dev - CUDU
$\bullet$ &  % C14n SW-ISX Prov
$\bullet$ &  % HW-ISX Prov
$\circ$ \\  % UE

&
raw data and algorithm knowledge &
$\circ$ & $\circ$ & $\bullet$  & $\circ$  &  % AKD
$\circ$ & $\circ$ & $\bullet$ & $\circ$ &  % AKM
$\circ$ & $\circ$ & $\circ$ & $\odot$ &  % ACD
$\circ$ & $\odot$ &  % ACM
$\circ$ & $\bullet$ & $\circ$ &  % AG
$\circ$ & $\circ$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-App Dev
$\bullet$ & $\bullet$ & $\circ$ & $\bullet$ & $\circ$ &  % O-RAN SW-ISX Dev - Non
$\circ$ & $\bullet$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-ISX Dev - Near
$\circ$ & $\circ$ & $\circ$ & $\bullet$ & $\bullet$ &  % O-RAN SW-ISX Dev - CUDU
$\bullet$ &  % C14n SW-ISX Prov
$\bullet$ &  % HW-ISX Prov
$\circ$ \\  % UE
&
data property and algorithm knowledge &
$\circ$ & $\circ$ & $\circ$  & $\bullet$  &  % AKD
$\circ$ & $\circ$ & $\bullet$ & $\circ$ &  % AKM
$\circ$ & $\circ$ & $\circ$ & $\odot$ &  % ACD
$\circ$ & $\odot$ &  % ACM
$\circ$ & $\bullet$ & $\circ$ &  % AG
$\circ$ & $\circ$ & $\bullet$ & $\bullet$ & $\circ$ &  % O-RAN SW-App Dev
$\bullet$ & $\bullet$ & $\circ$ & $\bullet$ & $\circ$ &  % O-RAN SW-ISX Dev - Non
$\circ$ & $\bullet$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-ISX Dev - Near
$\circ$ & $\circ$ & $\circ$ & $\bullet$ & $\bullet$ &  % O-RAN SW-ISX Dev - CUDU
$\bullet$ &  % C14n SW-ISX Prov
$\bullet$ &  % HW-ISX Prov
$\circ$ \\  % UE

&
training data and task knowledge &
$\bullet$ & $\circ$ & $\circ$  & $\circ$  &  % AKD
$\circ$ & $\circ$ & $\circ$ & $\bullet$ &  % AKM
$\circ$ & $\circ$ & $\circ$ & $\odot$ &  % ACD
$\circ$ & $\odot$ &  % ACM
$\circ$ & $\bullet$ & $\circ$ &  % AG
$\circ$ & $\circ$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-App Dev
$\bullet$ & $\bullet$ & $\circ$ & $\bullet$ & $\circ$ &  % O-RAN SW-ISX Dev - Non
$\bullet$ & $\bullet$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-ISX Dev - Near
$\circ$ & $\circ$ & $\circ$ & $\bullet$ & $\bullet$ &  % O-RAN SW-ISX Dev - CUDU
$\bullet$ &  % C14n SW-ISX Prov
$\bullet$ &  % HW-ISX Prov
$\circ$ \\  % UE

&
features data and task knowledge &
$\circ$ & $\bullet$ & $\circ$  & $\circ$  &  % AKD
$\circ$ & $\circ$ & $\circ$ & $\bullet$ &  % AKM
$\circ$ & $\circ$ & $\circ$ & $\odot$ &  % ACD
$\circ$ & $\odot$ &  % ACM
$\circ$ & $\bullet$ & $\circ$ &  % AG
$\circ$ & $\bullet$ & $\bullet$ & $\bullet$ & $\circ$ &  % O-RAN SW-App Dev
$\bullet$ & $\bullet$ & $\circ$ & $\bullet$ & $\circ$ &  % O-RAN SW-ISX Dev - Non
$\bullet$ & $\bullet$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-ISX Dev - Near
$\circ$ & $\circ$ & $\circ$ & $\bullet$ & $\bullet$ &  % O-RAN SW-ISX Dev - CUDU
$\bullet$ &  % C14n SW-ISX Prov
$\bullet$ &  % HW-ISX Prov
$\circ$ \\  % UE

&
raw data and task knowledge &
$\circ$ & $\circ$ & $\bullet$  & $\circ$  &  % AKD
$\circ$ & $\circ$ & $\circ$ & $\bullet$ &  % AKM
$\circ$ & $\circ$ & $\circ$ & $\odot$ &  % ACD
$\circ$ & $\odot$ &  % ACM
$\circ$ & $\bullet$ & $\circ$ &  % AG
$\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ &  % O-RAN SW-App Dev
$\bullet$ & $\bullet$ & $\circ$ & $\bullet$ & $\circ$ &  % O-RAN SW-ISX Dev - Non
$\bullet$ & $\bullet$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-ISX Dev - Near
$\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ &  % O-RAN SW-ISX Dev - CUDU
$\bullet$ &  % C14n SW-ISX Prov
$\bullet$ &  % HW-ISX Prov
$\circ$ \\  % UE

&
data property and task knowledge &
$\circ$ & $\circ$ & $\circ$  & $\bullet$  &  % AKD
$\circ$ & $\circ$ & $\circ$ & $\bullet$ &  % AKM
$\circ$ & $\circ$ & $\circ$ & $\odot$ &  % ACD
$\circ$ & $\odot$ &  % ACM
$\circ$ & $\bullet$ & $\circ$ &  % AG
$\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ &  % O-RAN SW-App Dev
$\bullet$ & $\bullet$ & $\circ$ & $\bullet$ & $\circ$ &  % O-RAN SW-ISX Dev - Non
$\bullet$ & $\bullet$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-ISX Dev - Near
$\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ &  % O-RAN SW-ISX Dev - CUDU
$\bullet$ &  % C14n SW-ISX Prov
$\bullet$ &  % HW-ISX Prov
$\circ$ \\  % UE
\Xhline{3\arrayrulewidth}

\multicolumn{42}{l}{Threat model -  \textbf{$\circ$}: does not require such type of access/knowledge, \textbf{$\bullet$}: such type of access/knowledge is required for generating the attack, \textbf{$\odot$}: such type of access/knowledge is required for executing the attack.} \\

\multicolumn{42}{l}{Impact -  \textbf{$\circ$}: The attacker can achieve such type of goal, by executing this attack, \textbf{$\bullet$}: The attacker can't achieve such type of goal, by executing this attack.} \\
\multicolumn{42}{l}{Threat Actor -  \textbf{$\bullet$}: The threat actor can obtain the capabilities required to execute the attack ,\textbf{$\circ$}:The threat actor cannot obtain the capabilities required to execute the attack.} \\

\end{tabular}}
\caption{Adversarial machine learning attack techniques and threat actors.}
\label{tab:attack_techniques_with_actors}
\end{table*}


==> sections/Tables/ahp_results.tex <==
\setlength\tabcolsep{4pt}
\begin{table*}[h!]
\scriptsize
\centering
\hspace*{-0.8cm}
\begin{tabular}{@{}
b{0.025\textwidth}|
b{0.025\textwidth}|
b{0.025\textwidth}|
b{0.025\textwidth}|
b{0.025\textwidth}|
b{0.025\textwidth}|
b{0.025\textwidth}|
b{0.025\textwidth}|
b{0.025\textwidth}|
b{0.025\textwidth}|
b{0.025\textwidth}"
b{0.025\textwidth}|
b{0.025\textwidth}|
b{0.025\textwidth}|
b{0.025\textwidth}|
b{0.025\textwidth}|
b{0.025\textwidth}|
b{0.025\textwidth}|
b{0.025\textwidth}"
b{0.025\textwidth}|
b{0.025\textwidth}|
b{0.025\textwidth}"
b{0.025\textwidth}|
b{0.025\textwidth}|
b{0.025\textwidth}|
b{0.025\textwidth}"
@{}}
\Xhline{3\arrayrulewidth}

\multicolumn{19}{c|}{Threat Model} & 
\multicolumn{3}{c|}{Attack Impact} &
\multicolumn{4}{c|}{Environmental Metrics} \\ \cline{1-19}

\multicolumn{11}{c"}{Access Capabilities} &
\multicolumn{8}{c"}{System Knowledge} & & & & & & & \\ \Xhline{3\arrayrulewidth}



\rotatebox{90}{Pipeline Access $[AC1]$} & 
\rotatebox{90}{Model Access $[AC2]$} & 
\rotatebox{90}{Prediction Access $[AC3]$} & 
\rotatebox{90}{Raw Data Access $[AC4]$} &
\rotatebox{90}{Training Data Access $[AC5]$} &
\rotatebox{90}{Labeled Data Access $[AC6]$} &
\rotatebox{90}{Validation Data Access $[AC7]$} &
\rotatebox{90}{Surrogate Data Access $[AC8]$} &
\rotatebox{90}{Score-Based Query Access $[AC9]$} &
\rotatebox{90}{Decision-Based Query Access $[AC10]$} &
\rotatebox{90}{Sensor Data Access $[AC11]$} &

\rotatebox{90}{Perfect Knowledge $[AK1]$} &
\rotatebox{90}{Model Knowledge $[AK2]$} &
\rotatebox{90}{Hyperparameter Knowledge $[AK3]$} &
\rotatebox{90}{Algorithm Knowledge $[AK4]$} &
\rotatebox{90}{Training Data Knowledge $[AK5]$} &
\rotatebox{90}{Raw Data Knowledge $[AK6]$} &
\rotatebox{90}{Data Property Knowledge $[AK7]$} &
\rotatebox{90}{Task Knowledge $[AK8]$} &

\rotatebox{90}{Tampering $[AG1]$} &
\rotatebox{90}{Denial of Service $[AG2]$} &
\rotatebox{90}{Information Disclosure $[AG3]$} &

\rotatebox{90}{Naive Pipeline} &
\rotatebox{90}{Pipeline With Data Validation} &
\rotatebox{90}{Pipeline With Feature Extraction} &
\rotatebox{90}{Pipeline With A/B Testing}

\\ \Xhline{3\arrayrulewidth}

\cellcolor{Grey} - &
\cellcolor{Low} 0.085 &
\cellcolor{VeryLow} 0.102 &
\cellcolor{VeryLow} 0.102 &
\cellcolor{VeryLow} 0.102 &
\cellcolor{VeryLow} 0.102 &
\cellcolor{VeryLow} 0.102 &
\cellcolor{Medium} 0.097 &
\cellcolor{High} 0.016 &
\cellcolor{High} 0.005 &
\cellcolor{High} 0.013 &
\cellcolor{Grey} - &
\cellcolor{Medium} 0.036 &
\cellcolor{High} 0.007 &
\cellcolor{High} 0.002 &
\cellcolor{Medium} 0.017 &
\cellcolor{VeryHigh} 0.001 &
\cellcolor{High} 0.004 &
\cellcolor{High} 0.003 &
\cellcolor{Medium} 0.022 &
\cellcolor{Medium} 0.022 &
\cellcolor{Medium} 0.022 &
\cellcolor{High} 0.007 &
\cellcolor{Low} 0.049 &
\cellcolor{VeryLow} 0.112 &
\cellcolor{Low} 0.049 \\  \Xhline{3\arrayrulewidth}


\end{tabular}%
\caption{Adversarial machine learning attack techniques.}
\label{tab:attack_techniques}
\end{table*}

==> sections/Tables/attack_D_table.tex <==
\setlength\tabcolsep{4.2pt}
\begin{table*}[h!]
\scriptsize
\centering
\hspace*{-1.5cm}
% \rotatebox{90}
%\resizebox{1.18\textwidth}{0.515\textheight}
{\begin{tabular}{|p{0.09\textwidth}"  % Threat Category
m{0.2\textwidth}"  % Attack Technique
m{0.425\textwidth}"  % Description
c"  % Phase
b{0.006\textwidth}|b{0.006\textwidth}|b{0.006\textwidth}|b{0.006\textwidth}|  % AKD
b{0.006\textwidth}|b{0.006\textwidth}|b{0.006\textwidth}|  % AKM
b{0.006\textwidth}|b{0.006\textwidth}|b{0.006\textwidth}|b{0.006\textwidth}|  % ACD
b{0.006\textwidth}|b{0.006\textwidth}"  % ACM
b{0.006\textwidth}|b{0.006\textwidth}|b{0.006\textwidth}|  % AG
% b{0.006\textwidth}"@{}
}
\Xhline{3\arrayrulewidth}

\multirow{4}{*}{\makecell{\textbf{Threat}\\\textbf{Category}}} &
\multirow{4}{*}{\textbf{Attack Technique}} &
\multirow{4}{*}{\textbf{Description}} &
\multirow{4}{*}{P} &
\multicolumn{16}{c|}{\textbf{Threat Model}} \\ 
\cline{5-20} 

& & & & 
\multicolumn{7}{c|}{Knowledge} &
\multicolumn{6}{c"}{Access} & 
\multicolumn{3}{c|}{Impact} \\ 
\cline{5-17}

& & & &
\multicolumn{4}{c|}{\makecell{AKD}} & 
\multicolumn{3}{c|}{\makecell{AKM}} & 
\multicolumn{4}{c|}{\makecell{ACD}} & 
\multicolumn{2}{c"}{\makecell{ACM}} & 
\multicolumn{3}{c|}{}\\ 
\cline{5-20}

& & & & 
% Data Knowledge
\rotatebox{90}{Training Data Knowledge} & 
\rotatebox{90}{Features Data Knowledge} & 
\rotatebox{90}{Raw Data Knowledge} & 
\rotatebox{90}{Data Property Knowledge} &

% Model Knowledge
\rotatebox{90}{Hyperparameter Knowledge} &
\rotatebox{90}{Algorithm Knowledge} &
\rotatebox{90}{Task Knowledge} &

% Data Access
\rotatebox{90}{Training Data Access} &
\rotatebox{90}{Features Data Access} &
\rotatebox{90}{Raw Data Access} &
\rotatebox{90}{Sensor Data Access} &

% Model Access
\rotatebox{90}{Score-Based Query Access} &
\rotatebox{90}{Decision-Based Query Access} &

% Impact
\rotatebox{90}{Tampering} &
\rotatebox{90}{Denial of Service} &
\rotatebox{90}{Information Disclosure} \\

\Xhline{3\arrayrulewidth}


% Evasion [T1]
\multirow{7}{*}{\textbf{Evasion}} &
Gradient-based, white-box, evasion attacks (C\&W \cite{carlini2017adversarial}, FGSM \cite{goodfellow2014explaining}, and BIM \cite{kurakin2016adversarial}) &
An adversary manipulates the input, using gradients calculations with respect to the input sample, to maximize the classification loss. &
\textbf{I} &
$\bullet$ & $\circ$ & $\circ$  & $\circ$ &  % AKD
$\bullet$ & $\circ$ & $\circ$ &  % AKM
$\circ$ & $\circ$ & $\circ$ & $\circ$ &  % ACD
$\circ$ & $\bullet$ &  % ACM
$\bullet$ & $\circ$ & $\circ$   % AG
\\ \cline{2-20}

&
Boundary-based, black-box (score-based), evasion attacks ( ZOO \cite{chen2017zoo}) &
An adversary manipulates the input to maximize the classification loss, using gradients estimations based on the model's probabilities vectors. &
\textbf{I} &
$\circ$ & $\circ$ & $\circ$  & $\circ$  &  % AKD
$\circ$ & $\circ$ & $\bullet$ &  % AKM
$\circ$ & $\circ$ & $\circ$ & $\circ$ &  % ACD
$\bullet$ & $\circ$ &  % ACM
$\bullet$ & $\circ$ & $\circ$  % AG
\\ \cline{2-20}

& 
Boundary-based, black-box (decision-based), evasion attacks ( HopSkipJump \cite{chen2020hopskipjumpattack}) &
An adversary manipulates the input to maximize the classification loss, using gradients estimations based on the model's decisions. &
\textbf{I} &
$\circ$ & $\circ$ & $\circ$  & $\circ$  &  % AKD
$\circ$ & $\circ$ & $\bullet$ &  % AKM
$\circ$ & $\circ$ & $\circ$ & $\circ$ &  % ACD
$\circ$ & $\bullet$ &  % ACM
$\bullet$ & $\circ$ & $\circ$ \\  % AG
\cline{2-20}

& 
Transferability-based, black-box (decision-based), evasion attacks that utilize reference data \cite{papernot2016transferability} &
An adversary manipulates the input to maximize the classification loss, using gradients calculations of a surrogate model trained on a reference data with similar characteristics and distribution as the training data. &
\textbf{I} &
$\circ$ & $\circ$ & $\circ$  & $\bullet$  &  % AKD
$\circ$ & $\circ$ & $\bullet$ &  % AKM
$\circ$ & $\circ$ & $\circ$ & $\circ$ &  % ACD
$\circ$ & $\bullet$ &  % ACM
$\bullet$ & $\circ$ & $\circ$ \\  % AG
\cline{2-20}

& 
Transferability-based, black-box (decision-based), evasion attacks that utilize training data ( \cite{papernot2016transferability}) &
An adversary manipulates the input to maximize the classification loss, using gradients calculations of a surrogate model trained on the same data used to train the target model. &
\textbf{I} &
$\bullet$ & $\circ$ & $\circ$  & $\circ$  &  % AKD
$\circ$ & $\circ$ & $\bullet$ &  % AKM
$\circ$ & $\circ$ & $\circ$ & $\circ$ &  % ACD
$\circ$ & $\odot$ &  % ACM
$\bullet$ & $\circ$ & $\circ$ \\  % AG
\cline{2-20}

& 
Gradient-based, targeted, white-box, poisoning attack (  \cite{kravchik2021poisoning,mei2015using,jagielski2018manipulating}) &
An adversary manipulates a small number of training samples to maximize the classification loss on other set of samples targeted by the attacker. The manipulation determined using gradients calculations of the target model. &
\textbf{T} &
$\bullet$ & $\circ$ & $\circ$  & $\circ$  &  % AKD
$\bullet$ & $\circ$ & $\circ$ &  % AKM
$\odot$ & $\circ$ & $\circ$ & $\circ$ &  % ACD
$\circ$ & $\odot$ &  % ACM
$\bullet$ & $\circ$ & $\circ$ \\  % AG
\cline{2-20}

&
Transferability-based, targeted, black-box, poisoning attack (error-specific or error generic  \cite{biggio2012poisoning,munoz2017towards,jagielski2018manipulating})) &
An adversary manipulates a small number of training samples to maximize the classification loss on other set of samples targeted by the attacker. The manipulation determined using gradients calculations of a surrogate model that trained on a reference data with similar characteristics and distribution as the target model's training data. &
\textbf{T} &
$\circ$ & $\circ$ & $\circ$  & $\bullet$  &  % AKD
$\circ$ & $\circ$ & $\bullet$ &  % AKM
$\odot$ & $\circ$ & $\circ$ & $\circ$ &  % ACD
$\circ$ & $\odot$ &  % ACM
$\bullet$ & $\circ$ & $\circ$ \\  % AG
\Xhline{3\arrayrulewidth}


% ML model corruption [T2]
\multirow{2}{*}{\makecell{\textbf{Model} \\ \textbf{Corruption}}} &
Gradient-based, indiscriminate, white-box poisoning attack ( \cite{kravchik2021poisoning,mei2015using,jagielski2018manipulating}) &
An adversary manipulates a small number of training samples to maximize the classification loss of an untainted dataset.
The manipulation determined using gradients calculations of the target model. &
\textbf{T} &
$\bullet$ & $\circ$ & $\circ$  & $\circ$  &  % AKD
$\bullet$ & $\circ$ & $\circ$ &  % AKM
$\odot$ & $\circ$ & $\circ$ & $\circ$ &  % ACD
$\circ$ & $\odot$ &  % ACM
$\bullet$ & $\bullet$ & $\circ$ \\  % AG
\cline{2-20}

&
Transferability-based, indiscriminate, black-box poisoning attack ( \cite{biggio2012poisoning,munoz2017towards,jagielski2018manipulating}) & 
An adversary manipulates a small number of training samples to maximize the classification loss of an untainted dataset.
The manipulation determined using gradients calculations of a surrogate model that trained on a reference data with similar characteristics and distribution as the target model's training data. &
\textbf{T} &
$\circ$ & $\circ$ & $\circ$  & $\bullet$  &  % AKD
$\circ$ & $\circ$ & $\bullet$ &  % AKM
$\odot$ & $\circ$ & $\circ$ & $\circ$ &  % ACD
$\circ$ & $\odot$ &  % ACM
$\bullet$ & $\bullet$ & $\circ$ \\  % AG
\Xhline{3\arrayrulewidth}


% Membership inference [T3]
\multirow{2}{*}{\makecell{\textbf{Membership} \\ \textbf{Inference}}} &
Shadow training-based, black-box membership inference attacks \cite{shokri2017membership} &
An adversary determine whether or not a given sample used to train the target model, based on shadow ML-model that classify whether or not the sample was part of the training set, given the target model's probabilities vector. &
\textbf{I} &
$\circ$ & $\circ$ & $\odot$  & $\circ$  &  % AKD
$\circ$ & $\circ$ & $\odot$ &  % AKM
$\circ$ & $\circ$ & $\circ$ & $\circ$ &  % ACD
$\bullet$ & $\circ$ &  % ACM
$\circ$ & $\circ$ & $\bullet$ \\  % AG
\cline{2-20}

&
Gradient-based, white-box membership inference attacks ( \cite{nasr2019comprehensive}) &
An adversary determine whether or not a given sample used to train the target model, based on the target model's gradients behavior during training. &
\textbf{T} &
$\odot$ & $\circ$ & $\circ$  & $\circ$  &  % AKD
$\bullet$ & $\circ$ & $\circ$ &  % AKM
$\odot$ & $\circ$ & $\circ$ & $\circ$ &  % ACD
$\circ$ & $\circ$ &  % ACM
$\circ$ & $\circ$ & $\bullet$ \\  % AG

\Xhline{3\arrayrulewidth}


% Data property inference [T4] 
\makecell{\textbf{Data Property} \\ \textbf{Inference}} &
Shadow training-based property inference attacks \cite{ateniese2015hacking,ganju2018property,song2020information} &
An adversary deduces a property of the training data using a shadow ML-model that classify whether or not the training data preserve the property, given the target model's probabilities vector. &
\textbf{I} &
$\odot$ & $\circ$ & $\circ$  & $\circ$  &  % AKD
$\circ$ & $\circ$ & $\odot$ &  % AKM
$\odot$ & $\circ$ & $\circ$ & $\circ$ &  % ACD
$\bullet$ & $\circ$ &  % ACM
$\circ$ & $\circ$ & $\bullet$ \\  % AG
\Xhline{3\arrayrulewidth}

% Data reconstruction (theft) [T5]
\multirow{3}{*}{\makecell{\textbf{Data} \\ \textbf{Reconstruction}}} &
Maximum a posteriori-based, gray-box data reconstruction attacks \cite{fredrikson2014privacy,hidano2017model} &
An adversary reconstruct samples from the training data along with their labels using maximum a posteriori estimation of the attribute that maximizes the probability of observing the known parameters while assuming partial access and knowledge of the target model and the training data. &
\textbf{I} &
$\odot$ & $\circ$ & $\circ$  & $\circ$  &  % AKD
$\bullet$ & $\circ$ & $\circ$ &  % AKM
$\odot$ & $\circ$ & $\circ$ & $\circ$ &  % ACD
$\bullet$ & $\circ$ &  % ACM
$\circ$ & $\circ$ & $\bullet$ \\  % AG
\cline{2-20}

&
Gradient optimization-based, gray-box data reconstruction attacks \cite{fredrikson2015model} &
An adversary reconstruct samples from the training data along with their labels by solving an optimization problem using gradient descent calculation on the target model to recover the input data point. &
\textbf{I} &
$\odot$ & $\circ$ & $\circ$  & $\circ$  &  % AKD
$\bullet$ & $\circ$ & $\circ$ &  % AKM
$\odot$ & $\circ$ & $\circ$ & $\circ$ &  % ACD
$\bullet$ & $\circ$ &  % ACM
$\circ$ & $\circ$ & $\bullet$ \\  % AG
\cline{2-20}

&
Black-box data reconstruction attacks \cite{yang2019neural} &
An adversary reconstruct samples from the training data along with their labels using an autoencoder settings where the target model plays the role of the encoder and the trainable decoder network tries to reconstruct the training sample from the target model's probabilities vector. &
\textbf{I} &
$\odot$ & $\circ$ & $\circ$  & $\circ$  &  % AKD
$\circ$ & $\circ$ & $\odot$ &  % AKM
$\odot$ & $\circ$ & $\circ$ & $\circ$ &  % ACD
$\bullet$ & $\circ$ &  % ACM
$\circ$ & $\circ$ & $\bullet$ \\  % AG
\Xhline{3\arrayrulewidth}

% Model Extraction [T6]
\makecell{\textbf{Model} \\ \textbf{Extraction}} &
Query-based, black-box model extraction attacks \cite{chandrasekaran2020exploring,juuti2019prada,oh2019towards,papernot2017practical} &
An adversary extract complete information of the target ML model by fully reconstructing it or creating a substitute model that behave very similarly using the target model's probabilities vector. &
\textbf{I} &
$\odot$ & $\circ$ & $\circ$  & $\circ$  &  % AKD
$\circ$ & $\circ$ & $\odot$ &  % AKM
$\circ$ & $\circ$ & $\circ$ & $\circ$ &  % ACD
$\bullet$ & $\circ$ &  % ACM
$\circ$ & $\circ$ & $\bullet$ \\  % AG
\Xhline{3\arrayrulewidth}


% Resource Exhaustion [T7]
\multirow{3}{*}{\makecell{\textbf{Resource} \\ \textbf{Exhaustion}}} &
White-box Sponge examples \cite{shumailov2020sponge} &
An adversary manipulates the input, using gradients calculations of the target model, to maximize the model latency or energy consumption. &
\textbf{I} &
$\circ$ & $\circ$ & $\circ$  & $\circ$  &  % AKD
$\bullet$ & $\circ$ & $\circ$ &  % AKM
$\circ$ & $\circ$ & $\circ$ & $\circ$ &  % ACD
$\circ$ & $\bullet$ &  % ACM
$\circ$ & $\bullet$ & $\circ$ \\  % AG
\cline{2-20}

&
Interactive black-box sponge examples \cite{shumailov2020sponge} &
An adversary manipulates the input, using gradients estimations based on the target model's probabilities vector, to maximize the model latency or energy consumption. &
\textbf{I} &
$\circ$ & $\circ$ & $\circ$  & $\circ$  &  % AKD
$\odot$ & $\circ$ & $\circ$ &  % AKM
$\circ$ & $\circ$ & $\circ$ & $\circ$ &  % ACD
$\circ$ & $\bullet$ &  % ACM
$\circ$ & $\bullet$ & $\circ$ \\  % AG
\cline{2-20}

&
Blind black-box sponge example and hardware transferability \cite{shumailov2020sponge} &
An adversary manipulates the input, using gradients calculations of a surrogate model, to maximize the model latency or energy consumption. &
\textbf{I} &
$\circ$ & $\circ$ & $\circ$  & $\odot$  &  % AKD
$\circ$ & $\circ$ & $\odot$ &  % AKM
$\circ$ & $\circ$ & $\circ$ & $\circ$ &  % ACD
$\circ$ & $\bullet$ &  % ACM
$\circ$ & $\bullet$ & $\circ$ \\  % AG
\Xhline{3\arrayrulewidth}

\multicolumn{20}{l}{Attack phase -  \textbf{I}: inference, \textbf{T}: training.}\\

\multicolumn{20}{l}{Access capabilities -  \textbf{$\circ$}: does not require such type of access, \textbf{$\odot$}: limited access of such type is required , \textbf{$\bullet$}: complete access of such type is required.} \\


\multicolumn{20}{l}{System knowledge -  \textbf{$\circ$}: does not require such type of knowledge,$\odot$: require partial knowledge \textbf{$\bullet$}: require full knowledge.} \\
\multicolumn{20}{l}{Attack Goal -  \textbf{$\circ$}: The attacker can achieve such type of goal, by executing this attack, \textbf{$\bullet$}: The attacker can't achieve such type of goal, by executing this attack.} \\

\end{tabular}}
\caption{Adversarial machine learning attack techniques.}
\label{tab:attack_techniques}
\end{table*}

==> sections/Tables/attack_table.tex <==
\setlength\tabcolsep{4.2pt}
\begin{table*}[h!]
\scriptsize
\centering
\hspace*{-1.3cm}
\begin{tabular}{@{}l"m{0.27\textwidth}|c|c"b{0.003\textwidth}|b{0.01\textwidth}|b{0.006\textwidth}|b{0.006\textwidth}|b{0.006\textwidth}|b{0.006\textwidth}|b{0.006\textwidth}|b{0.006\textwidth}|b{0.006\textwidth}|b{0.006\textwidth}"b{0.006\textwidth}|b{0.005\textwidth}|b{0.006\textwidth}|b{0.006\textwidth}|b{0.006\textwidth}|b{0.006\textwidth}|b{0.006\textwidth}|b{0.006\textwidth}"b{0.006\textwidth}|b{0.006\textwidth}|b{0.006\textwidth}|b{0.015\textwidth}|@{}}
\Xhline{3\arrayrulewidth}

\multirow{3}{*}{Threat Category} &
\multirow{3}{*}{Attack Technique} &
\multirow{3}{*}{Target Assets} &
\multirow{3}{*}{P} &
\multicolumn{21}{c|}{Threat Model} & 
\multirow{3}{*}{S}  \\ \cline{5-25} 

& & & & 
\multicolumn{10}{c"}{Access Capabilities} &
\multicolumn{8}{c"}{System Knowledge} & 
\multicolumn{3}{c|}{Goal} & \\ \cline{5-25}

& & & & 
\rotatebox{90}{Pipeline Access $[AC1]$} & 
\rotatebox{90}{Model Access $[AC2]$} & 
\rotatebox{90}{Prediction Access $[AC3]$} & 
\rotatebox{90}{Raw Data Access $[AC4]$} &
\rotatebox{90}{Training Data Access $[AC5]$} &
\rotatebox{90}{Labeled Data Access $[AC6]$} &
\rotatebox{90}{Validation Data Access $[AC7]$} &
\rotatebox{90}{Surrogate Data Access $[AC8]$} &
\rotatebox{90}{Score-Based Query Access $[AC9]$} &
\rotatebox{90}{Decision-Based Query Access $[AC10]$} &

\rotatebox{90}{Perfect Knowledge $[AK1]$} &
\rotatebox{90}{Model Knowledge $[AK2]$} &
\rotatebox{90}{Hyperparameter Knowledge $[AK3]$} &
\rotatebox{90}{Algorithm Knowledge $[AK4]$} &
\rotatebox{90}{Training Data Knowledge $[AK5]$} &
\rotatebox{90}{Raw Data Knowledge $[AK6]$} &
\rotatebox{90}{Data Property Knowledge $[AK7]$} &
\rotatebox{90}{Task Knowledge $[AK8]$} &

\rotatebox{90}{Tampering $[AG1]$} &
\rotatebox{90}{Denial of Service $[AG2]$} &
\rotatebox{90}{Information Disclosure $[AG3]$} &

\\ \Xhline{3\arrayrulewidth}

% \textit{[T1]} Evading an ML system
\multirow{9}{*}{\makecell{\textbf{Evasion} \\ \textbf{\textit{[T1]}}}}  &
Gradient-based, white-box, evasion attacks (such as C\&W \cite{carlini2017adversarial}) FGSM \cite{goodfellow2014explaining}, and BIM \cite{kurakin2016adversarial}) &
$[A9]$ Model&
\textbf{I}&
$\circ$ & $\circ$ & $\circ$  & $\circ$  & $\circ$ & $\circ$ & $\circ$ & $\circ$ & $\circ$ & $\circ$ &
$\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ &
$\bullet$ & $\circ$  & $\circ$ & \cellcolor{High} 8.3 \\ \cline{2-25}

&
Boundary-based, black-box (score-based), evasion attacks (such as ZOO \cite{chen2017zoo})&
$[A9]$ Model&
\textbf{I}&
$\circ$ & $\circ$ & $\circ$  & $\circ$  & $\circ$ & $\circ$ & $\circ$ & $\circ$ & $\bullet$ & $\circ$ &
$\circ$ & $\circ$ & $\circ$ & $\circ$ & $\circ$ & $\circ$ & $\circ$ & $\bullet$ &
$\bullet$ & $\circ$  & $\circ$ & \cellcolor{VeryHigh} 9 \\ \cline{2-25}

&
Boundary-based, black-box (decision-based), evasion attacks (such as HopSkipJump \cite{chen2020hopskipjumpattack})&
$[A9]$ Model&
\textbf{I}&
$\circ$ & $\circ$ & $\circ$  & $\circ$  & $\circ$ & $\circ$ & $\circ$ & $\circ$ & $\circ$ & $\bullet$ &
$\circ$ & $\circ$ & $\circ$ & $\circ$ & $\circ$ & $\circ$ & $\circ$ & $\bullet$ &
$\bullet$ & $\circ$  & $\circ$ & \cellcolor{VeryHigh} 9.1  \\ \cline{2-25}

&
Transferability-based, black-box (decision-based), evasion attacks that utilize reference data (such as Jacobian Data Augmentation \cite{papernot2016transferability})&
$[A9]$ Model&
\textbf{I}&
$\circ$ & $\circ$ & $\circ$  & $\circ$  & $\circ$ & $\circ$ & $\circ$ & $\odot$ & $\circ$ & $\bullet$ &
$\circ$ & $\circ$ & $\circ$ & $\circ$ & $\circ$ & $\circ$ & $\bullet$ & $\bullet$ &
$\bullet$ & $\circ$  & $\circ$  & \cellcolor{VeryHigh} 9 \\ \cline{2-25}

&
Transferability-based, black-box (decision-based), evasion attacks that utilize training data (such as \cite{papernot2016transferability})&
$[A9]$ Model&
\textbf{I}&
$\circ$ & $\circ$ & $\circ$  & $\circ$  & $\circ$ & $\circ$ & $\circ$ &  $\circ$ & $\circ$ & $\bullet$ &
$\circ$ & $\circ$ & $\circ$ & $\circ$ & $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ &
$\bullet$ & $\circ$  & $\circ$  & \cellcolor{Medium} 7.6 \\ \cline{2-25}

&
Gradient-based, targeted, white-box, poisoning attack (such as  \cite{kravchik2021poisoning,mei2015using,jagielski2018manipulating})&
$[A9]$ Model&
\textbf{T}&
$\circ$ & $\circ$ & $\circ$  & $\odot$  & $\odot$ & $\odot$ & $\circ$ & $\circ$ & $\circ$ &$\odot$ &
$\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ &
$\bullet$ & $\circ$  & $\circ$  & \cellcolor{VeryLow} 4.7\\ \cline{2-25}

&
Transferability-based, targeted, black-box, poisoning attack (error-specific or error generic such as \cite{biggio2012poisoning,munoz2017towards,jagielski2018manipulating}))&
$[A9]$ Model&

\textbf{T}&
$\circ$ & $\circ$ & $\circ$  & $\odot$  & $\odot$ & $\odot$ & $\circ$ &  $\bullet$ & $\circ$ &$\odot$ &
$\circ$ & $\circ$ & $\circ$ & $\circ$ & $\bullet$ & $\circ$ & $\bullet$ & $\bullet$ &
$\bullet$ & $\circ$  & $\circ$  & \cellcolor{Low} 5.1 \\ \cline{2-25}

&
Gradient-based, targeted, white-box, poisoning attack against feature selection (such as \cite{xiao2015feature})&
$[A7]$ Feature selection&
\textbf{T}&
$\circ$ & $\circ$ & $\circ$  & $\odot$  & $\odot$ & $\odot$ & $\circ$ & $\circ$ & $\circ$ &$\odot$ &
$\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ &
$\bullet$ & $\circ$  & $\circ$  & \cellcolor{VeryLow} 4.7  \\ \cline{2-25}

&
Transferability-based, targeted, black-box, poisoning attack against feature selection (such as \cite{xiao2015feature})&
$[A7]$ Feature selection&
\textbf{T}&
$\circ$ & $\circ$ & $\circ$  & $\odot$  & $\odot$ & $\odot$ & $\circ$ &  $\bullet$ & $\circ$ &$\odot$ &
$\circ$ & $\circ$ & $\circ$ & $\circ$ & $\bullet$ & $\circ$ & $\bullet$ & $\bullet$ &
$\bullet$ & $\circ$  & $\circ$  & \cellcolor{Low} 5.1  \\ \Xhline{3\arrayrulewidth}

% \textit{[T2]} ML model corruption

\multirow{4}{*}{\makecell{\textbf{ML model corruption} \\ \textbf{\textit{[T2]}}}} &
Gradient-based, indiscriminate, white-box poisoning attack (such as \cite{kravchik2021poisoning,mei2015using,jagielski2018manipulating})&
$[A9]$ Model&

\textbf{T}&
$\circ$ & $\circ$ & $\circ$  & $\odot$  & $\odot$ & $\odot$ & $\circ$ & $\circ$ & $\circ$ &$\odot$ &
$\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ &
$\bullet$ & $\bullet$  & $\circ$  & \cellcolor{VeryLow} 4.7 \\ \cline{2-25}


&
Transferability-based, indiscriminate, black-box poisoning attack (such as \cite{biggio2012poisoning,munoz2017towards,jagielski2018manipulating})&
$[A9]$ Model&

\textbf{T}&
$\circ$ & $\circ$ & $\circ$  & $\odot$  & $\odot$ & $\odot$ & $\circ$ &  $\bullet$ & $\circ$ &$\odot$ &
$\circ$ & $\circ$ & $\circ$ & $\circ$ & $\bullet$ & $\circ$ & $\bullet$ & $\bullet$ &
$\bullet$ & $\bullet$  & $\circ$  & \cellcolor{Low} 5.4 \\ \cline{2-25}

&
Gradient-based, indiscriminate, white-box poisoning attack against feature selection (such as \cite{xiao2015feature})&
$[A7]$ Feature selection&
\textbf{T}&
$\circ$ & $\circ$ & $\circ$  & $\odot$  & $\odot$ & $\odot$ & $\circ$ & $\circ$ & $\circ$ &$\odot$ &
$\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ &
$\bullet$ & $\bullet$  & $\circ$   & \cellcolor{VeryLow} 4.7 \\ \cline{2-25}

&
Transferability-based, indiscriminate, black-box poisoning attack against feature selection (such as \cite{xiao2015feature})&
$[A7]$ Feature selection&
\textbf{T}&
$\circ$ & $\circ$ & $\circ$  & $\odot$  & $\odot$ & $\odot$ & $\circ$ &  $\bullet$ & $\circ$ &$\odot$ &
$\circ$ & $\circ$ & $\circ$ & $\circ$ & $\bullet$ & $\circ$ & $\bullet$ & $\bullet$ &
$\bullet$ & $\bullet$  & $\circ$  & \cellcolor{Low} 5.4 \\ \Xhline{3\arrayrulewidth}

%\textit{[T3]} Membership inference}

\multirow{3}{*}{\makecell{\textbf{Membership inference} \\ \textbf{\textit{[T3]}}}}&
Shadow training-based, black-box membership inference attacks \cite{shokri2017membership}&
\makecell{ $[A1]$ Data lake  \\ $[A5]$ Feature store }&

\textbf{I}&
$\circ$ & $\circ$ & $\circ$  & $\odot$  & $\odot$ & $\circ$ & $\circ$ & $\circ$ & $\bullet$ & $\bullet$ &
$\circ$ & $\circ$ & $\circ$ & $\circ$ & $\odot$ & $\circ$ & $\circ$ & $\bullet$ &
$\circ$ & $\circ$  & $\bullet$  & \cellcolor{VeryHigh} 8.9 \\ \cline{2-25}


&
Gradient-based, white-box membership inference attacks (such as \cite{nasr2019comprehensive})&
\makecell{ $[A1]$ Data lake  \\ $[A5]$ Feature store }&

\textbf{T}&
$\circ$ & $\bullet$ & $\bullet$  & $\odot$  & $\odot$ & $\circ$ & $\circ$ & $\circ$ & $\bullet$ & $\circ$ &
$\circ$ & $\bullet$ & $\bullet$ & $\bullet$ & $\odot$ & $\circ$ & $\circ$ & $\bullet$ &
$\circ$ & $\circ$  & $\bullet$  & \cellcolor{High} 8.3 \\ \cline{2-25}

&
Membership inference attacks exploiting attacker's access &
\makecell{ $[A1]$ Data lake  \\ $[A5]$ Feature store }&

\textbf{I}&
$\circ$ & $\circ$ & $\circ$  & $\bullet$  & $\bullet$ & $\bullet$ & $\circ$ & $\circ$ & $\circ$ & $\circ$ &
$\circ$ & $\circ$ & $\circ$ & $\circ$ & $\circ$ & $\circ$ & $\circ$ & $\circ$ &
$\circ$ & $\circ$  & $\bullet$  & \cellcolor{Low} 5.5 \\ \Xhline{3\arrayrulewidth}

%\textit{[T4]} Data property inference} 
\multirow{2}{*}{\makecell{\textbf{Data property inference} \\ \textbf{\textit{[T4]}}}}&
Shadow training-based property inference attacks \cite{ateniese2015hacking,ganju2018property,song2020information}&
\makecell{ $[A1]$ Data lake  \\ $[A5]$ Feature store }&

\textbf{I}&
$ \circ $ & $ \circ $ & $ \circ $  & $ \odot $  & $ \odot $ & $ \circ $ & $ \circ $ & $ \circ $ & $ \bullet $ & $ \bullet $ &
$ \circ $ & $ \circ $ & $ \circ $ & $ \circ $ & $ \odot $ & $ \circ $ & $ \circ $ & $ \odot $ &
$ \circ $ & $ \circ $  & $ \bullet $  & \cellcolor{VeryHigh} 8.9  \\ 
\cline{2-25}

&
Property inference attacks exploiting attacker's access &
\makecell{ $[A1]$ Data lake  \\ $[A5]$ Feature store }&

\textbf{I}&
$\circ$ & $\circ$ & $\circ$  & $\bullet$  & $\bullet$ & $\bullet$ & $\circ$ & $\circ$ & $\circ$ & $\circ$ &
$\circ$ & $\circ$ & $\circ$ & $\circ$ & $\circ$ & $\circ$ & $\circ$ & $\circ$ &
$\circ$ & $\circ$  & $\bullet$  & \cellcolor{Low} 5.5  \\ \Xhline{3\arrayrulewidth}

% \textbf{\textit{[T4]} Data property inference} &
% White-box property inference attacks \cite{}&
% 
% \textbf{I}&
% $ \circ $ & $ \bullet $ & $ \bullet $  & $ \odot $  & $ \odot $ & $ \circ $ & $ \circ $ & $ \odot $ & $ \bullet $ & $ \bullet $ &
% $ \odot $ & $ \bullet $ & $ \bullet $ & $ \bullet $ & $ \odot $ & $ \circ $ & $ \circ $ & $ \odot $ &
% $ \circ $ & $ \circ $  & $ \bullet $ \\ \hline

%\textit{[T5]} Data reconstruction (theft)

\multirow{4}{*}{\makecell{\textbf{Data reconstruction} \\ \textbf{\textit{[T5]}}}} &
Maximum a posteriori-based, gray-box data reconstruction attacks \cite{fredrikson2014privacy,hidano2017model}&
\makecell{ $[A1]$ Data lake  \\ $[A5]$ Feature store }&

\textbf{I}&
$\circ$ & $\odot$ & $\odot$  & $\odot$  & $\odot$ & $\circ$ & $\circ$ & $\circ$ & $\bullet$ & $\bullet$ &
$\circ$ & $\bullet$ & $\circ$ & $\circ$ & $\odot$ & $\odot$ & $\circ$ & $\odot$ &
$\circ$ & $\circ$  & $\bullet$  & \cellcolor{High} 8.4 \\ \cline{2-25}

&
Gradient optimization-based, gray-box data reconstruction attacks \cite{fredrikson2015model}&
\makecell{ $[A1]$ Data lake  \\ $[A5]$ Feature store }&

\textbf{I}&
$\circ$ & $\odot$ & $\odot$  & $\odot$  & $\odot$ & $\circ$ & $\circ$ & $\circ$ & $\bullet$ & $\bullet$ &
$\circ$ & $\bullet$ & $\circ$ & $\circ$ & $\odot$ & $\odot$ & $\circ$ & $\odot$ &
$\circ$ & $\circ$  & $\bullet$ & \cellcolor{High} 8.4 \\ \cline{2-25}

&
Black-box data reconstruction attacks \cite{yang2019neural}&
\makecell{ $[A1]$ Data lake  \\ $[A5]$ Feature store }&

\textbf{I}&
$ \circ $ & $ \circ $ & $ \circ $  & $ \odot $  & $ \odot $ & $ \circ $ & $ \circ $ & $ \circ $ & $ \bullet $ & $ \bullet $ &
$ \circ $ & $ \circ $ & $ \circ $ & $ \circ $ & $ \odot $ & $ \odot $ & $ \circ $ & $ \odot $ &
$ \circ $ & $ \circ $  & $ \bullet $ & \cellcolor{VeryHigh} 8.9 \\ \cline{2-25}


&
Data theft due to data breach &
\makecell{ $[A1]$ Data lake  \\ $[A5]$ Feature store }&

\textbf{I}&
$\circ$ & $\circ$ & $\circ$  & $\bullet$  & $\bullet$ & $\bullet$ & $\circ$ & $\circ$ & $\circ$ & $\circ$ &
$\circ$ & $\circ$ & $\circ$ & $\circ$ & $\circ$ & $\circ$ & $\circ$ & $\circ$ &
$\circ$ & $\circ$  & $\bullet$ & \cellcolor{Low} 5.5 \\ \Xhline{3\arrayrulewidth}

\multirow{2}{*}{\makecell{\textbf{Model extraction} \\ \textbf{\textit{[T6]}}}} &
Query-based, black-box model extraction attacks \cite{chandrasekaran2020exploring,juuti2019prada,oh2019towards,papernot2017practical}&
$[A9]$ Model&

\textbf{I}&
$\circ$ & $\circ$ & $\circ$  & $\circ$  & $\circ$ & $\circ$ & $\circ$ & $\circ$ & $\bullet$ & $\bullet$ &
$\circ$ & $\circ$ & $\circ$ & $\circ$ & $\odot$ & $\odot$ & $\circ$ & $\odot$ &
$\circ$ & $\circ$  & $\bullet$ & \cellcolor{VeryHigh} 9.1\\ \cline{2-25}


&
Attacker's access-based model extraction attack &
$[A9]$ Model&

\textbf{I}&
$\circ$ & $\bullet$ & $\circ$  & $\circ$  & $\circ$ & $\circ$ & $\circ$ & $\circ$ & $\circ$ & $\circ$ &
$\circ$ & $\circ$ & $\circ$ & $\circ$ & $\circ$ & $\circ$ & $\circ$ & $\circ$ &
$\circ$ & $\circ$  & $\bullet$  & \cellcolor{Low} 5.5\\ \Xhline{3\arrayrulewidth}


\multicolumn{25}{l}{Attack phase -  \textbf{I}: inference, \textbf{T}: training.}\\

\multicolumn{25}{l}{Access capabilities -  \textbf{$\circ$}: does not require such type of access
 , \textbf{$\odot$}: limited access of such type is required , \textbf{$\bullet$}: complete access of such type is required.} \\


\multicolumn{25}{l}{System knowledge -  \textbf{$\circ$}: does not require such type of knowledge,$\odot$: require partial knowledge \textbf{$\bullet$}: require full knowledge.} \\
\multicolumn{25}{l}{Attack Goal -  \textbf{$\circ$}: The attacker can achieve such type of goal, by executing this attack, \textbf{$\bullet$}: The attacker can't achieve such type of goal, by executing this attack.} \\


\end{tabular}%
\caption{Adversarial machine learning attack techniques.}
\label{tab:attack_techniques}
\end{table*}

==> sections/Tables/ml_func_2_oran_components.tex <==
% \begin{tabular}[c]{|>{\centering}m{0.24\textwidth}">{\centering}p{0.13\textwidth}|>{\centering}p{0.18\textwidth}|>{\centering}p{0.18\textwidth}|p{0.18\textwidth}|}
%     \Xhline{3\arrayrulewidth}
%     \multirow{2}{*}{AI/ML Functionalities} & \multirow{2}{*}{Type} & \multirow{2}{*}{High Latency} & \multicolumn{2}{c|}{Low Latency} \\
%     \cline{4-5}
%     & & & Supervised \& Unsupervised Learning & Reinforcement \& Online Learning \\
%     \Xhline{3\arrayrulewidth}
%     \begin{tabular}[c]{@{}c@{}}Data Lake \\ {[}F1{]}\end{tabular} & Shared Data Layer API (SDL) & \nonrt & \nonrt & \nrt \\ \hline
%     \begin{tabular}[c]{@{}c@{}}Data Host\\ {[}F2{]}\end{tabular} & xApp / rApp & on the training and inference hosts in the \nonrt & on the training host in the \nonrt~and on the inference host in the \nrt & on the training and inference hosts in the \nrt \\ \hline
%     \begin{tabular}[c]{@{}c@{}}Feature Store \\ {[}F3{]}\end{tabular} & xApp / rApp & on the training and inference hosts in the \nonrt & on the training host in the \nonrt~and on the inference host in the \nrt & on the training and inference hosts in the \nrt \\ \hline
%     \begin{tabular}[c]{@{}c@{}}Training Host \\ {[}F4{]}\end{tabular} & xApp / rApp & on the training host in the \nonrt & on the training host in the \nonrt & on the training host in the \nrt \\ \hline
%     \begin{tabular}[c]{@{}c@{}}Model Catalog \\ {[}F5{]}\end{tabular} & Shared Data Layer API (SDL) & \nonrt & \nonrt & \nrt \\ \hline
%     \begin{tabular}[c]{@{}c@{}}Model\\ {[}F6{]}\end{tabular} & Static file (e.g. h5, pickle) & on the inference host in the \nonrt & on the inference host in the \nrt & on the inference host in the \nrt \\ \hline
%     \begin{tabular}[c]{@{}c@{}}Model Serving\\ {[}F7{]}\end{tabular} & 
%     xApp / rApp / app's supplier's servers & 
%     on the training host in the \nonrt~/ on the app's supplier's servers & 
%     on the training host in the \nonrt~/on the app's supplier's servers & 
%     on the training host in the \nrt \\ \hline
%     \begin{tabular}[c]{@{}c@{}}\mlaa \\ {[}F8{]}\end{tabular} & Shared Data Layer API (SDL) & \nonrt & \nonrt & \nrt \\ \hline
    
%      & & & & \\ \hline
     
%     Example Use-Case & - & 
%     NSSI Resource Allocation & 
%     Traffic Steering & 
%     Context Based Dynamic Handover Management for V2X \\ \hline
%     \end{tabular}

% ------------------------------------

% -----------------------------------

\begin{tabular}[c]{|>{\centering}m{0.24\textwidth}">{\centering}p{0.13\textwidth}|>{\centering}p{0.18\textwidth}|>{\centering}p{0.18\textwidth}|p{0.12\textwidth}|}
    \Xhline{3\arrayrulewidth}
    \multirow{2}{*}{AI/ML Functionalities} & \multirow{2}{*}{Type} & \multirow{2}{*}{High Latency} & \multicolumn{2}{c|}{Low Latency} \\
    \cline{4-5}
    & & & Supervised \& Unsupervised Learning & Reinforcement \& Online Learning \\
    \Xhline{3\arrayrulewidth}
    \begin{tabular}[c]{@{}c@{}}Data Lake \\ {[}F1{]}\end{tabular} & Shared Data Layer API (SDL) & \nonrt & \nonrt & \nrt \\ 
    \hline
    \begin{tabular}[c]{@{}c@{}}Data Host\\ {[}F2{]}\end{tabular} & xApp / rApp & \nonrt & during the training phase in the \nonrt and during the serving phase in the \nrt & \nrt \\ \hline
    \begin{tabular}[c]{@{}c@{}}Feature Store \\ {[}F3{]}\end{tabular} & Shared Data Layer API (SDL) & \nonrt & during the training phase in the \nonrt and during the serving phase in the \nrt & \nrt \\ 
    \hline
    \begin{tabular}[c]{@{}c@{}}Training Host \\ {[}F4{]}\end{tabular} & xApp / rApp & \nonrt & \nonrt & \nrt \\ 
    \hline
    \begin{tabular}[c]{@{}c@{}}Model Catalog \\ {[}F5{]}\end{tabular} & Shared Data Layer API (SDL) & \nonrt & \nrt & \nrt \\ 
    \hline
    \begin{tabular}[c]{@{}c@{}}Model\\ {[}F6{]}\end{tabular} & Static file (e.g. h5, pickle) & \nonrt & \nrt & \nrt \\ 
    \hline
    \begin{tabular}[c]{@{}c@{}}Model Serving\\ {[}F7{]}\end{tabular} & 
    xApp / rApp & \nonrt & \nrt & \nrt \\ 
    \hline
    \begin{tabular}[c]{@{}c@{}}\mlaa \\ {[}F8{]}\end{tabular} & xApp / rApp & \nonrt & \nrt & \nrt \\ 
    \hline
    
     & & & & \\ \hline
     
    Example Use-Case & - & 
    NSSI Resource Allocation & 
    Traffic Steering & 
    Context Based Dynamic HO Management for V2X \\ \hline
    \end{tabular}

==> sections/Tables/ml_func_to_oran_cmp.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\newcommand{\latencyDepend}{\nrt~/ \nonrt~(latency dependant).}
\newcommand{\latencyDependExt}{O-DU / O-CU / \nrt~/ \nonrt~(latency dependant).}
% \begin{table*}[h]
% \small
% \centering

\begin{tabular}{|c"p{0.15\textwidth}|p{0.16\textwidth}|p{0.17\textwidth}|p{0.17\textwidth}|}
\Xhline{3\arrayrulewidth}
\multirow{2}{*}{AI/ML Functionalities} & \multirow{2}{*}{Type} & \multicolumn{3}{c|}{ML Task} \\ \cline{3-5}
 & & \rotatebox[]{90}{Supervised}& \rotatebox[]{90}{Unsupervised} & \rotatebox[]{90}{Reinforcement Learning}\\
\Xhline{3\arrayrulewidth}
% \begin{tabular}[c]{@{}c@{}}\textbf{\textit{Example Component}} \\ \textbf{\textit{{[}A0{]}}}\end{tabular} & \textbf{\textit{static file/procedures/servers}}  & \textbf{\textit{where in supervised}} & \textbf{\textit{where in unsupervised}} & \textbf{\textit{where in reinforcement}}\\ \hline

\begin{tabular}[c]{@{}c@{}}Data Lake \\ {[}A1{]}\end{tabular} & Servers. Access via Shared Data Layer API (SDL)  & \nonrt & \nonrt & \latencyDepend\\ \hline
\begin{tabular}[c]{@{}c@{}}Data Extraction\\ {[}A2{]}\end{tabular} & Servers. Access via SDL & \nonrt & \nonrt & \latencyDepend\\ \hline
\begin{tabular}[c]{@{}c@{}}Data Validation\\ {[}A3{]}\end{tabular} & Servers. Access via SDL & \nonrt & \nonrt & \latencyDepend\\ \hline
\begin{tabular}[c]{@{}c@{}}Data Preparation\\ {[}A4{]}\end{tabular} & Servers. Access via SDL & \nonrt & \nonrt & \latencyDepend\\ \hline
\begin{tabular}[c]{@{}c@{}}Feature Store\\ {[}A5{]}\end{tabular} & Servers. Access via SDL & \nonrt & \nonrt & \latencyDepend\\ \hline
\begin{tabular}[c]{@{}c@{}}Data Labeling\\ {[}A6{]}\end{tabular} & \dan{Comp.} & \dan{Comp.} & \dan{Comp.} & \dan{Comp.} \\ \hline
\begin{tabular}[c]{@{}c@{}}Feature Selection\\ {[}A7{]}\end{tabular} & Servers. Access via SDL & \nonrt & \nonrt & \latencyDepend\\ \hline
\begin{tabular}[c]{@{}c@{}}Model Training\\ {[}A8{]}\end{tabular} & Procedure. & \nonrt & \nonrt & \latencyDepend \\ \hline
\begin{tabular}[c]{@{}c@{}}Model\\ {[}A9{]}\end{tabular} & Static file(e.g. h5, pickle) & \latencyDependExt & \latencyDependExt & \latencyDependExt \\ \hline
\begin{tabular}[c]{@{}c@{}}Model Repository\\ {[}A10{]}\end{tabular} & Servers. & \nonrt & \nonrt & \nonrt \\ \hline
\begin{tabular}[c]{@{}c@{}}Model Evaluation\\ {[}A11{]}\end{tabular} & Servers. & \nonrt &\nonrt &\nonrt \\ \hline
\begin{tabular}[c]{@{}c@{}}Model Offline Validation\\ {[}A12{]}\end{tabular} & Servers. & \nonrt & \nonrt & \nonrt \\ \hline
\begin{tabular}[c]{@{}c@{}}Model Online Validation\\ {[}A13{]}\end{tabular} & Servers. & \nonrt & \nonrt & \nonrt \\ \hline
\begin{tabular}[c]{@{}c@{}}Model Serving\\ {[}A14{]}\end{tabular} & Servers. & \latencyDependExt & \latencyDependExt & \latencyDependExt \\ \hline
\begin{tabular}[c]{@{}c@{}}Model Performance Monitoring\\ {[}A15{]}\end{tabular} & Servers. & \nonrt & \nonrt & \latencyDepend \\

\Xhline{3\arrayrulewidth}

\end{tabular}
% \caption{AI/ML Workflow components Deployment in \oran }
% \label{tab:aiml_dep}
% \end{table*}

==> sections/Tables/old_Attack_Table_with_Actors.tex <==
\setlength\tabcolsep{4.2pt}
\begin{table*}[h!]
\scriptsize
\centering
\hspace*{-1.5cm}
% \rotatebox{90}
\resizebox{1.15\textwidth}{0.515\textheight}
{\begin{tabular}{@{}
|p{0.075\textwidth}"  % Threat Category
m{0.18\textwidth}"  % Attack Technique
% c"  % P
p{0.0005\textwidth}"  % P
b{0.005\textwidth}|b{0.005\textwidth}|b{0.005\textwidth}|b{0.005\textwidth}|  % AKD
b{0.005\textwidth}|b{0.005\textwidth}|b{0.005\textwidth}|  % AKM
b{0.005\textwidth}|b{0.005\textwidth}|b{0.005\textwidth}|b{0.005\textwidth}|  % ACD
b{0.005\textwidth}|b{0.005\textwidth}"  % ACM
b{0.005\textwidth}|b{0.005\textwidth}|b{0.005\textwidth}"  % AG
% ||b{0.005\textwidth}|  % Help Titles
b{0.005\textwidth}|b{0.005\textwidth}|b{0.005\textwidth}|b{0.005\textwidth}|b{0.005\textwidth}"  % SW App Dev
b{0.005\textwidth}|b{0.005\textwidth}|b{0.005\textwidth}|b{0.005\textwidth}|b{0.005\textwidth}"  % SW ISX Dev-nonRT
b{0.005\textwidth}|b{0.005\textwidth}|b{0.005\textwidth}|b{0.005\textwidth}|b{0.005\textwidth}"  % SW ISX Dev-nRT
b{0.005\textwidth}|b{0.005\textwidth}|b{0.005\textwidth}|b{0.005\textwidth}|b{0.005\textwidth}"  % SW ISX Dev-CUDU
p{0.033\textwidth}"  % Contatiner SW ISX Prov
b{0.033\textwidth}"  % HW ISX Prov
b{0.034\textwidth}|  % UE
% @{}  % Last col space=0
}
\Xhline{3\arrayrulewidth}

\multirow{5}{*}{\makecell{\textbf{Threat}\\\textbf{Category}}} &
\multirow{5}{*}{\textbf{Attack Technique}} &
\multirow{5}{*}{\textbf{P}} &
\multicolumn{16}{c"}{\textbf{Threat Model}} & 
\multicolumn{23}{c|}{\textbf{Threat Actor}} \\
\cline{4-42} 

& & & 
\multicolumn{7}{c|}{Knowledge} &
\multicolumn{6}{c"}{Access} & 
\multicolumn{3}{c"}{Impact} & 
\multicolumn{5}{c"}{\textbf{\textit{[TAi1]}} } &  % O-RAN SW-App Dev
\multicolumn{15}{c"}{\textbf{\textit{[TAi2]}} } &  % O-RAN SW-ISX Dev
\textbf{\textit{[TAi3]}} &  % Containerization SW-ISX Prov
\textbf{\textit{[TAi4]}} &  % HW-IDX Prov
\textbf{\textit{[TAe1]}} \\  % UE
\cline{4-16} \cline{20-42}

& & &
\multicolumn{4}{c|}{AKD} &  % Knowledge
\multicolumn{3}{c|}{AKM} &  % Knowledge
\multicolumn{4}{c|}{ACD} &  % Access
\multicolumn{2}{c"}{ACM} &  % Access
\multicolumn{3}{c"}{ } &  % Impace
\rotatebox{90}{Data Collection} &  % SW-App Dev
\rotatebox{90}{Data Host} &  % SW-App Dev
\rotatebox{90}{Training Host} &  % SW-App Dev
\rotatebox{90}{Serving Host} &  % SW-App Dev
\rotatebox{90}{ML App} &  % SW-App Dev
\multicolumn{5}{c"}{\makecell{Non-RT\\RIC}} &  % SW-ISX Dev
\multicolumn{5}{c"}{\makecell{Near-RT\\RIC}} &  % SW-ISX Dev
\multicolumn{5}{c"}{\makecell{O-CU / \\O-DU}} &  % SW-ISX Dev
\makecell{All} &  % C14n SW-ISX Prov
\makecell{All} &  % HW-ISX Prov
\makecell{All} \\  % UE
\cline{4-42}

& & & 
% Data Knowledge
\rotatebox{90}{Training Data Knowledge} & 
\rotatebox{90}{Features Data Knowledge} & 
\rotatebox{90}{Raw Data Knowledge} & 
\rotatebox{90}{Data Property Knowledge} &

% Model Knowledge
\rotatebox{90}{Hyperparameter Knowledge} &
\rotatebox{90}{Algorithm Knowledge} &
\rotatebox{90}{Task Knowledge} &

% Data Access
\rotatebox{90}{Training Data Access} &
\rotatebox{90}{Features Data Access} &
\rotatebox{90}{Raw Data Access} &
\rotatebox{90}{Sensor Data Access} &

% Model Access
\rotatebox{90}{Score-Based Query Access} &
\rotatebox{90}{Decision-Based Query Access} &

% Impact
\rotatebox{90}{Tampering} &
\rotatebox{90}{Denial of Service} &
\rotatebox{90}{Information Disclosure} & 

% O-RAN SW-App Dev (DS)
\multicolumn{5}{c"}{\rotatebox{90}{\makecell{All \\Deployment \\Scenarios}}} & 

% O-RAN SW-ISX Dev (DS)
\rotatebox{90}{\textit{DS 1}} & \rotatebox{90}{\textit{DS 2}} & \rotatebox{90}{\textit{DS 3}} & \rotatebox{90}{\textit{DS 4}} & \rotatebox{90}{\textit{DS 5}} &  %  Non-RT RIC
\rotatebox{90}{\textit{DS 1}} & \rotatebox{90}{\textit{DS 2}} & \rotatebox{90}{\textit{DS 3}} & \rotatebox{90}{\textit{DS 4}} & \rotatebox{90}{\textit{DS 5}} &  %  Near-RT RIC
\rotatebox{90}{\textit{DS 1}} & \rotatebox{90}{\textit{DS 2}} & \rotatebox{90}{\textit{DS 3}} & \rotatebox{90}{\textit{DS 4}} & \rotatebox{90}{\textit{DS 5}} &  %  O-CU/O-DU
All &  % C14n SW-IDX Prov
All &  % HW-IDX Prov
All \\  % UE
\Xhline{3\arrayrulewidth}


% Evasion [T1]
\multirow{7}{*}{\textbf{Evasion}} 

&
Gradient-based, white-box, evasion attacks (C\&W \cite{carlini2017adversarial}, FGSM \cite{goodfellow2014explaining}, and BIM \cite{kurakin2016adversarial}) &
\textbf{I} &
$\bullet$ & $\circ$ & $\circ$  & $\circ$ &  % AKD
$\bullet$ & $\circ$ & $\circ$ &  % AKM
$\circ$ & $\circ$ & $\circ$ & $\circ$ &  % ACD
$\circ$ & $\bullet$ &  % ACM
$\bullet$ & $\circ$ & $\circ$ &  % AG
$\circ$ & $\circ$ & $\bullet$ & $\bullet$ & $\circ$ &  % O-RAN SW-App Dev
$\bullet$ & $\bullet$ & $\circ$ & $\bullet$ & $\circ$ &  % O-RAN SW-ISX Dev - Non
$\circ$ & $\bullet$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-ISX Dev - Near
$\circ$ & $\circ$ & $\circ$ & $\bullet$ & $\bullet$ &  % O-RAN SW-ISX Dev - CUDU
$\bullet$ &  % C14n SW-ISX Prov
$\bullet$ &  % HW-ISX Prov
$\circ$ \\  % UE
\cline{2-42}

&
Boundary-based, black-box (score-based), evasion attacks ( ZOO \cite{chen2017zoo}) &
\textbf{I} &
$\circ$ & $\circ$ & $\circ$  & $\circ$  &  % AKD
$\circ$ & $\circ$ & $\bullet$ &  % AKM
$\circ$ & $\circ$ & $\circ$ & $\circ$ &  % ACD
$\bullet$ & $\circ$ &  % ACM
$\bullet$ & $\circ$ & $\circ$ &  % AG
$\circ$ & $\circ$ & $\bullet$ & $\bullet$ & $\bullet$ &  % O-RAN SW-App Dev
$\bullet$ & $\bullet$ & $\circ$ & $\bullet$ & $\circ$ &  % O-RAN SW-ISX Dev - Non
$\bullet$ & $\bullet$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-ISX Dev - Near
$\circ$ & $\circ$ & $\circ$ & $\bullet$ & $\bullet$ &  % O-RAN SW-ISX Dev - CUDU
$\bullet$ &  % C14n SW-ISX Prov
$\bullet$ &  % HW-ISX Prov
$\circ$ \\  % UE
\cline{2-42}

& 
Boundary-based, black-box (decision-based), evasion attacks ( HopSkipJump \cite{chen2020hopskipjumpattack}) &
\textbf{I} &
$\circ$ & $\circ$ & $\circ$  & $\circ$  &  % AKD
$\circ$ & $\circ$ & $\bullet$ &  % AKM
$\circ$ & $\circ$ & $\circ$ & $\circ$ &  % ACD
$\circ$ & $\bullet$ &  % ACM
$\bullet$ & $\circ$ & $\circ$ &  % AG
$\circ$ & $\circ$ & $\bullet$ & $\bullet$ & $\bullet$ &  % O-RAN SW-App Dev
$\bullet$ & $\bullet$ & $\circ$ & $\bullet$ & $\circ$ &  % O-RAN SW-ISX Dev - Non
$\bullet$ & $\bullet$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-ISX Dev - Near
$\circ$ & $\circ$ & $\circ$ & $\bullet$ & $\bullet$ &  % O-RAN SW-ISX Dev - CUDU
$\bullet$ &  % C14n SW-ISX Prov
$\bullet$ &  % HW-ISX Prov
$\bullet$ \\  % UE
\cline{2-42}

& 
Transferability-based, black-box (decision-based), evasion attacks that utilize reference data \cite{papernot2016transferability} &
\textbf{I} &
$\circ$ & $\circ$ & $\circ$  & $\bullet$  &  % AKD
$\circ$ & $\circ$ & $\bullet$ &  % AKM
$\circ$ & $\circ$ & $\circ$ & $\circ$ &  % ACD
$\circ$ & $\bullet$ &  % ACM
$\bullet$ & $\circ$ & $\circ$ &  % AG
$\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ &  % O-RAN SW-App Dev
$\bullet$ & $\bullet$ & $\circ$ & $\bullet$ & $\circ$ &  % O-RAN SW-ISX Dev - Non
$\bullet$ & $\bullet$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-ISX Dev - Near
$\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ &  % O-RAN SW-ISX Dev - CUDU
$\bullet$ &  % C14n SW-ISX Prov
$\bullet$ &  % HW-ISX Prov
$\odot$ \\  % UE
\cline{2-42}

& 
Transferability-based, black-box (decision-based), evasion attacks that utilize training data ( \cite{papernot2016transferability}) &
\textbf{I} &
$\bullet$ & $\circ$ & $\circ$  & $\circ$  &  % AKD
$\circ$ & $\circ$ & $\bullet$ &  % AKM
$\circ$ & $\circ$ & $\circ$ & $\circ$ &  % ACD
$\circ$ & $\odot$ &  % ACM
$\bullet$ & $\circ$ & $\circ$ &  % AG
$\circ$ & $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ &  % O-RAN SW-App Dev
$\bullet$ & $\bullet$ & $\circ$ & $\bullet$ & $\circ$ &  % O-RAN SW-ISX Dev - Non
$\bullet$ & $\bullet$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-ISX Dev - Near
$\circ$ & $\circ$ & $\circ$ & $\bullet$ & $\bullet$ &  % O-RAN SW-ISX Dev - CUDU
$\bullet$ &  % C14n SW-ISX Prov
$\bullet$ &  % HW-ISX Prov
$\circ$ \\  % UE
\cline{2-42}

& 
Gradient-based, targeted, white-box, poisoning attack (  \cite{kravchik2021poisoning,mei2015using,jagielski2018manipulating}) &
\textbf{T} &
$\bullet$ & $\circ$ & $\circ$  & $\circ$  &  % AKD
$\bullet$ & $\circ$ & $\circ$ &  % AKM
$\odot$ & $\circ$ & $\circ$ & $\circ$ &  % ACD
$\circ$ & $\odot$ &  % ACM
$\bullet$ & $\circ$ & $\circ$ &  % AG
$\circ$ & $\circ$ & $\bullet$ & $\bullet$ & $\circ$ &  % O-RAN SW-App Dev
$\bullet$ & $\bullet$ & $\circ$ & $\bullet$ & $\circ$ &  % O-RAN SW-ISX Dev - Non
$\circ$ & $\bullet$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-ISX Dev - Near
$\circ$ & $\circ$ & $\circ$ & $\bullet$ & $\bullet$ &  % O-RAN SW-ISX Dev - CUDU
$\bullet$ &  % C14n SW-ISX Prov
$\bullet$ &  % HW-ISX Prov
$\circ$ \\  % UE
\cline{2-42}

&
Transferability-based, targeted, black-box, poisoning attack (error-specific or error generic  \cite{biggio2012poisoning,munoz2017towards,jagielski2018manipulating})) &
\textbf{T} &
$\circ$ & $\circ$ & $\circ$  & $\bullet$  &  % AKD
$\circ$ & $\circ$ & $\bullet$ &  % AKM
$\odot$ & $\circ$ & $\circ$ & $\circ$ &  % ACD
$\circ$ & $\odot$ &  % ACM
$\bullet$ & $\circ$ & $\circ$ &  % AG
$\odot$ & $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ &  % O-RAN SW-App Dev
$\bullet$ & $\bullet$ & $\circ$ & $\bullet$ & $\circ$ &  % O-RAN SW-ISX Dev - Non
$\bullet$ & $\bullet$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-ISX Dev - Near
$\odot$ & $\odot$ & $\odot$ & $\bullet$ & $\bullet$ &  % O-RAN SW-ISX Dev - CUDU
$\bullet$ &  % C14n SW-ISX Prov
$\bullet$ &  % HW-ISX Prov
$\circ$ \\  % UE
\Xhline{3\arrayrulewidth}


% ML model corruption [T2]
\multirow{2}{*}{\makecell{\textbf{Model} \\ \textbf{Corruption}}} 

&
Gradient-based, indiscriminate, white-box poisoning attack ( \cite{kravchik2021poisoning,mei2015using,jagielski2018manipulating}) &
\textbf{T} &
$\bullet$ & $\circ$ & $\circ$  & $\circ$  &  % AKD
$\bullet$ & $\circ$ & $\circ$ &  % AKM
$\odot$ & $\circ$ & $\circ$ & $\circ$ &  % ACD
$\circ$ & $\odot$ &  % ACM
$\bullet$ & $\bullet$ & $\circ$ &  % AG
$\circ$ & $\bullet$ & $\bullet$ & $\bullet$ & $\circ$ &  % O-RAN SW-App Dev
$\bullet$ & $\bullet$ & $\circ$ & $\bullet$ & $\circ$ &  % O-RAN SW-ISX Dev - Non
$\bullet$ & $\bullet$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-ISX Dev - Near
$\circ$ & $\circ$ & $\circ$ & $\bullet$ & $\bullet$ &  % O-RAN SW-ISX Dev - CUDU
$\bullet$ &  % C14n SW-ISX Prov
$\bullet$ &  % HW-ISX Prov
$\circ$ \\  % UE
\cline{2-42}

&
Transferability-based, indiscriminate, black-box poisoning attack ( \cite{biggio2012poisoning,munoz2017towards,jagielski2018manipulating}) & 
\textbf{T} &
$\circ$ & $\circ$ & $\circ$  & $\bullet$  &  % AKD
$\circ$ & $\circ$ & $\bullet$ &  % AKM
$\odot$ & $\circ$ & $\circ$ & $\circ$ &  % ACD
$\circ$ & $\odot$ &  % ACM
$\bullet$ & $\bullet$ & $\circ$ &  % AG
$\odot$ & $\bullet$ & $\bullet$ & $\bullet$ & $\circ$ &  % O-RAN SW-App Dev
$\bullet$ & $\bullet$ & $\circ$ & $\bullet$ & $\circ$ &  % O-RAN SW-ISX Dev - Non
$\bullet$ & $\bullet$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-ISX Dev - Near
$\odot$ & $\odot$ & $\odot$ & $\bullet$ & $\bullet$ &  % O-RAN SW-ISX Dev - CUDU
$\bullet$ &  % C14n SW-ISX Prov
$\bullet$ &  % HW-ISX Prov
$\circ$ \\  % UE
\Xhline{3\arrayrulewidth}


% Membership inference [T3]
\multirow{2}{*}{\makecell{\textbf{Membership} \\ \textbf{Inference}}} 

&
Shadow training-based, black-box membership inference attacks \cite{shokri2017membership} &
\textbf{I} &
$\circ$ & $\circ$ & $\odot$  & $\circ$  &  % AKD
$\circ$ & $\circ$ & $\odot$ &  % AKM
$\circ$ & $\circ$ & $\circ$ & $\circ$ &  % ACD
$\bullet$ & $\circ$ &  % ACM
$\circ$ & $\circ$ & $\bullet$ &  % AG
$\circ$ & $\circ$ & $\bullet$ & $\bullet$ & $\bullet$ &  % O-RAN SW-App Dev
$\bullet$ & $\bullet$ & $\circ$ & $\bullet$ & $\circ$ &  % O-RAN SW-ISX Dev - Non
$\bullet$ & $\bullet$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-ISX Dev - Near
$\circ$ & $\circ$ & $\circ$ & $\bullet$ & $\bullet$ &  % O-RAN SW-ISX Dev - CUDU
$\bullet$ &  % C14n SW-ISX Prov
$\bullet$ &  % HW-ISX Prov
$\circ$ \\  % UE
\cline{2-42}

&
Gradient-based, white-box membership inference attacks ( \cite{nasr2019comprehensive}) &
\textbf{T} &
$\odot$ & $\circ$ & $\circ$  & $\circ$  &  % AKD
$\bullet$ & $\circ$ & $\circ$ &  % AKM
$\odot$ & $\circ$ & $\circ$ & $\circ$ &  % ACD
$\circ$ & $\circ$ &  % ACM
$\circ$ & $\circ$ & $\bullet$ &  % AG
$\circ$ & $\circ$ & $\bullet$ & $\bullet$ & $\circ$ &  % O-RAN SW-App Dev
$\bullet$ & $\bullet$ & $\circ$ & $\bullet$ & $\circ$ &  % O-RAN SW-ISX Dev - Non
$\circ$ & $\bullet$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-ISX Dev - Near
$\circ$ & $\circ$ & $\circ$ & $\bullet$ & $\bullet$ &  % O-RAN SW-ISX Dev - CUDU
$\bullet$ &  % C14n SW-ISX Prov
$\bullet$ &  % HW-ISX Prov
$\circ$ \\  % UE
\Xhline{3\arrayrulewidth}


% Data property inference [T4] 
\makecell{\textbf{Data Property} \\ \textbf{Inference}} 

&
Shadow training-based property inference attacks \cite{ateniese2015hacking,ganju2018property,song2020information} &
\textbf{I} &
$\odot$ & $\circ$ & $\circ$  & $\circ$  &  % AKD
$\circ$ & $\circ$ & $\odot$ &  % AKM
$\odot$ & $\circ$ & $\circ$ & $\circ$ &  % ACD
$\bullet$ & $\circ$ &  % ACM
$\circ$ & $\circ$ & $\bullet$ &  % AG
$\circ$ & $\circ$ & $\bullet$ & $\bullet$ & $\bullet$ &  % O-RAN SW-App Dev
$\bullet$ & $\bullet$ & $\circ$ & $\bullet$ & $\circ$ &  % O-RAN SW-ISX Dev - Non
$\bullet$ & $\bullet$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-ISX Dev - Near
$\circ$ & $\circ$ & $\circ$ & $\bullet$ & $\bullet$ &  % O-RAN SW-ISX Dev - CUDU
$\bullet$ &  % C14n SW-ISX Prov
$\bullet$ &  % HW-ISX Prov
$\circ$ \\  % UE
\Xhline{3\arrayrulewidth}

% Data reconstruction (theft) [T5]
\multirow{3}{*}{\makecell{\textbf{Data} \\ \textbf{Reconstruction}}} 

&
Maximum a posteriori-based, gray-box data reconstruction attacks \cite{fredrikson2014privacy,hidano2017model} &
\textbf{I} &
$\odot$ & $\circ$ & $\circ$  & $\circ$  &  % AKD
$\bullet$ & $\circ$ & $\circ$ &  % AKM
$\odot$ & $\circ$ & $\circ$ & $\circ$ &  % ACD
$\bullet$ & $\circ$ &  % ACM
$\circ$ & $\circ$ & $\bullet$ &  % AG
$\circ$ & $\circ$ & $\bullet$ & $\bullet$ & $\circ$ &  % O-RAN SW-App Dev
$\bullet$ & $\bullet$ & $\circ$ & $\bullet$ & $\circ$ &  % O-RAN SW-ISX Dev - Non
$\circ$ & $\bullet$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-ISX Dev - Near
$\circ$ & $\circ$ & $\circ$ & $\bullet$ & $\bullet$ &  % O-RAN SW-ISX Dev - CUDU
$\bullet$ &  % C14n SW-ISX Prov
$\bullet$ &  % HW-ISX Prov
$\circ$ \\  % UE
\cline{2-42}

&
Gradient optimization-based, gray-box data reconstruction attacks \cite{fredrikson2015model} &
\textbf{I} &
$\odot$ & $\circ$ & $\circ$  & $\circ$  &  % AKD
$\bullet$ & $\circ$ & $\circ$ &  % AKM
$\odot$ & $\circ$ & $\circ$ & $\circ$ &  % ACD
$\bullet$ & $\circ$ &  % ACM
$\circ$ & $\circ$ & $\bullet$ &  % AG
$\circ$ & $\circ$ & $\bullet$ & $\bullet$ & $\circ$ &  % O-RAN SW-App Dev
$\bullet$ & $\bullet$ & $\circ$ & $\bullet$ & $\circ$ &  % O-RAN SW-ISX Dev - Non
$\circ$ & $\bullet$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-ISX Dev - Near
$\circ$ & $\circ$ & $\circ$ & $\bullet$ & $\bullet$ &  % O-RAN SW-ISX Dev - CUDU
$\bullet$ &  % C14n SW-ISX Prov
$\bullet$ &  % HW-ISX Prov
$\circ$ \\  % UE
\cline{2-42}

&
Black-box data reconstruction attacks \cite{yang2019neural} &
\textbf{I} &
$\odot$ & $\circ$ & $\circ$  & $\circ$  &  % AKD
$\circ$ & $\circ$ & $\odot$ &  % AKM
$\odot$ & $\circ$ & $\circ$ & $\circ$ &  % ACD
$\bullet$ & $\circ$ &  % ACM
$\circ$ & $\circ$ & $\bullet$ &  % AG
$\circ$ & $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ &  % O-RAN SW-App Dev
$\bullet$ & $\bullet$ & $\circ$ & $\bullet$ & $\circ$ &  % O-RAN SW-ISX Dev - Non
$\bullet$ & $\bullet$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-ISX Dev - Near
$\circ$ & $\circ$ & $\circ$ & $\bullet$ & $\bullet$ &  % O-RAN SW-ISX Dev - CUDU
$\bullet$ &  % C14n SW-ISX Prov
$\bullet$ &  % HW-ISX Prov
$\circ$ \\  % UE
\Xhline{3\arrayrulewidth}

% Model Extraction [T6]
\makecell{\textbf{Model} \\ \textbf{Extraction}} 

&
Query-based, black-box model extraction attacks \cite{chandrasekaran2020exploring,juuti2019prada,oh2019towards,papernot2017practical} &
\textbf{I} &
$\odot$ & $\circ$ & $\circ$  & $\circ$  &  % AKD
$\circ$ & $\circ$ & $\odot$ &  % AKM
$\circ$ & $\circ$ & $\circ$ & $\circ$ &  % ACD
$\bullet$ & $\circ$ &  % ACM
$\circ$ & $\circ$ & $\bullet$ &  % AG
$\circ$ & $\circ$ & $\bullet$ & $\bullet$ & $\bullet$ &  % O-RAN SW-App Dev
$\bullet$ & $\bullet$ & $\circ$ & $\bullet$ & $\circ$ &  % O-RAN SW-ISX Dev - Non
$\bullet$ & $\bullet$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-ISX Dev - Near
$\circ$ & $\circ$ & $\circ$ & $\bullet$ & $\bullet$ &  % O-RAN SW-ISX Dev - CUDU
$\bullet$ &  % C14n SW-ISX Prov
$\bullet$ &  % HW-ISX Prov
$\circ$ \\  % UE
\Xhline{3\arrayrulewidth}


% Resource Exhaustion [T7]
\multirow{3}{*}{\makecell{\textbf{Resource} \\ \textbf{Exhaustion}}} 

&
White-box Sponge examples \cite{shumailov2020sponge} &
\textbf{I} &
$\circ$ & $\circ$ & $\circ$  & $\circ$  &  % AKD
$\bullet$ & $\circ$ & $\circ$ &  % AKM
$\circ$ & $\circ$ & $\circ$ & $\circ$ &  % ACD
$\circ$ & $\bullet$ &  % ACM
$\circ$ & $\bullet$ & $\circ$ &  % AG
$\circ$ & $\circ$ & $\bullet$ & $\bullet$ & $\circ$ &  % O-RAN SW-App Dev
$\bullet$ & $\bullet$ & $\circ$ & $\bullet$ & $\circ$ &  % O-RAN SW-ISX Dev - Non
$\circ$ & $\bullet$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-ISX Dev - Near
$\circ$ & $\circ$ & $\circ$ & $\bullet$ & $\bullet$ &  % O-RAN SW-ISX Dev - CUDU
$\bullet$ &  % C14n SW-ISX Prov
$\bullet$ &  % HW-ISX Prov
$\circ$ \\  % UE
\cline{2-42}

&
Interactive black-box sponge examples \cite{shumailov2020sponge} &
\textbf{I} &
$\circ$ & $\circ$ & $\circ$  & $\circ$  &  % AKD
$\odot$ & $\circ$ & $\circ$ &  % AKM
$\circ$ & $\circ$ & $\circ$ & $\circ$ &  % ACD
$\circ$ & $\bullet$ &  % ACM
$\circ$ & $\bullet$ & $\circ$ &  % AG
$\odot$ & $\circ$ & $\bullet$ & $\bullet$ & $\bullet$ &  % O-RAN SW-App Dev
$\bullet$ & $\bullet$ & $\circ$ & $\bullet$ & $\circ$ &  % O-RAN SW-ISX Dev - Non
$\bullet$ & $\bullet$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-ISX Dev - Near
$\odot$ & $\odot$ & $\odot$ & $\bullet$ & $\bullet$ &  % O-RAN SW-ISX Dev - CUDU
$\bullet$ &  % C14n SW-ISX Prov
$\bullet$ &  % HW-ISX Prov
$\odot$ \\  % UE
\cline{2-42}

&
Blind black-box sponge example and hardware transferability \cite{shumailov2020sponge} &
\textbf{I} &
$\circ$ & $\circ$ & $\circ$  & $\odot$  &  % AKD
$\circ$ & $\circ$ & $\odot$ &  % AKM
$\circ$ & $\circ$ & $\circ$ & $\circ$ &  % ACD
$\circ$ & $\bullet$ &  % ACM
$\circ$ & $\bullet$ & $\circ$ &  % AG
$\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ &  % O-RAN SW-App Dev
$\bullet$ & $\bullet$ & $\circ$ & $\bullet$ & $\circ$ &  % O-RAN SW-ISX Dev - Non
$\bullet$ & $\bullet$ & $\bullet$ & $\circ$ & $\circ$ &  % O-RAN SW-ISX Dev - Near
$\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ &  % O-RAN SW-ISX Dev - CUDU
$\bullet$ &  % C14n SW-ISX Prov
$\bullet$ &  % HW-ISX Prov
$\bullet$ \\  % UE
\Xhline{3\arrayrulewidth}

\multicolumn{42}{l}{Attack phase -  \textbf{I}: inference, \textbf{T}: training.}\\

\multicolumn{42}{l}{Access capabilities -  \textbf{$\circ$}: does not require such type of access, \textbf{$\odot$}: limited access of such type is required , \textbf{$\bullet$}: complete access of such type is required.} \\


\multicolumn{42}{l}{System knowledge -  \textbf{$\circ$}: does not require such type of knowledge,$\odot$: require partial knowledge \textbf{$\bullet$}: require full knowledge.} \\
\multicolumn{42}{l}{Attack Goal -  \textbf{$\circ$}: The attacker can achieve such type of goal, by executing this attack, \textbf{$\bullet$}: The attacker can't achieve such type of goal, by executing this attack.} \\

\end{tabular}}
\caption{Adversarial Machine Learning Attack Techniques and Threat Actors.}
\label{tab:attack_techniques_with_actors}
\end{table*}

==> sections/Tables/research_vs_production.tex <==
\begin{table*}[h!]
\scriptsize
\centering
\begin{tabular}{@{}l"c|c|c"c|c|c|c|c|c|c|c"b{0.003\textwidth}|b{0.003\textwidth}|b{0.003\textwidth}|b{0.003\textwidth}|b{0.003\textwidth}|@{}}
\Xhline{3\arrayrulewidth}
& Data & Deployment & Orchestration & \multicolumn{8}{c"}{Pipeline} & \multicolumn{5}{c|}{Delivery} \\ \cline{5-17} 
& & & &\rotatebox{90}{Data Extraction} & \rotatebox{90}{Data Analysis} & \rotatebox{90}{Data Validation} & \rotatebox{90}{Data Preparation}& \rotatebox{90}{Model Training} & \rotatebox{90}{Model Offline Evaluation} & \rotatebox{90}{Model Offline Validation} & \rotatebox{90}{Model Online Validation} & \rotatebox{90}{Continuous Model Retraining} & \rotatebox{90}{Performance Monitoring} & \rotatebox{90}{Feature Store} & \rotatebox{90}{Model Registry} & \rotatebox{90}{Model Serving} \\ \Xhline{3\arrayrulewidth}
\textbf{Research}    & Offline & Single Host & Manual & $\bullet$ & $\bullet$ & $\circ$  & $\bullet$  & $\bullet$ & $\bullet$ & $\bullet$ & $\circ$ & $\circ$ & $\circ$ & $\circ$ & $\circ$ & $\circ$ \\
\hline
\textbf{Production} & Online  & Cluster & Automated & $\bullet$ & $\circ$ & $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ \\ \Xhline{3\arrayrulewidth}
\end{tabular}%
\caption{A comparison of the main characteristics and components of machine learning research and production workflows.}
\label{tab:r_p_cmp}
\end{table*}


==> sections/Tables/threat_model_inf_soft_dev.tex <==
\begin{table*}[t]
\small
    \centering
    \begin{tabular}{
    |c|c|c|c|c|c|
    }
     \hline
   \makecell{DC} & DS & \makecell{Data\\Knowledge} & \makecell{Model\\Knowledge} & \makecell{Data\\Access} & \makecell{Model\\Access}  \\ \hline
  
  \multirow{5}{*}{\makecell{Non\\Real\\Time\\RIC}} & 1 & Training Data  & Hyperparameter  & Training Data  & Score\\
  & 2 & Training Data  & Hyperparameter  & Training Data  & - \\
  & 3 & - & - & - & - \\
  & 4 & Training Data  & Hyperparameter  & Training Data  & - \\
  & 5 & - & - & - & - \\ \hline
  
  \multirow{5}{*}{\makecell{Near\\Real\\Time\\RIC}} & 1 & Features Data  & - & - & Score\\
   & 2 & Features Data  & Hyperparameter  & Feature Data  & Score\\
   & 3 & Training Data  & Hyperparameter  & Training Data  & Score\\
   & 4 & - & - & - & - \\
   & 5 & - & - & - & - \\ \hline
  
  \multirow{5}{*}{\makecell{O-CU\\O-DU}}  & 1 & Raw Data& - & Raw Data& - \\
  & 2 & Raw Data & - & Raw Data & - \\
  & 3 & Raw Data & - & Raw Data & - \\
  & 4 & Feature Data & Hyperparameter & Feature Data & Score\\
  & 5 & Training Data & Hyperparameter & Training Data & Score\\ \hline
  
  \multicolumn{6}{l}{DC - Developed Component, DS - Deployment Scenario} \\ 
 
\end{tabular}
    \caption{The adversarial capabilities of infrastructure software developer (Please note that due to space limitation we state the most severe capability according to Figure ~\ref{fig:adversarial_capabilities})}
    \label{tab:inf_soft_dev}
\end{table*}

==> sections/Tables/threat_model_soft_dev.tex <==
\begin{table}[t]
\scriptsize
    \centering
    \begin{tabular}{
    |p{0.095\textwidth}|p{0.085\textwidth}|p{0.095\textwidth}|p{0.085\textwidth}|p{0.04\textwidth}|
    }\hline
   \makecell{Developed\\Application} & \makecell{Data\\Knowledge} & \makecell{Model\\Knowledge} & \makecell{Data\\Access} & \makecell{Model\\Access}\\ \hline
   
   Data Collection & Raw Data & - & Raw Data & - \\ \hline
   
   Data Host & Features Data & - & Feature Data & - \\ \hline
   
   Training Host & Training Data & Hyperparameter & Training Data & - \\ \hline
   
   Serving Host & Features Data & Hyperparameter & Feature Data & Score \\ \hline
   
   ML APP Host & - & Task & - & Score \\ \hline
    
\end{tabular}
    \caption{The adversarial capabilities of software developer (Please note that due to space limitation we state the most severe capability according to Figure ~\ref{fig:adversarial_capabilities})}
    \label{tab:soft_dev}
\end{table}
